Householder QR Factorization with Randomization for Column Pivoting (HQRRP). FLAME Working Note #78

A fundamental problem when adding column pivoting to the Householder QR factorization is that only about half of the computation can be cast in terms of high performing matrix-matrix multiplications, which greatly limits the benefits that can be derived from so-called blocking of algorithms. This paper describes a technique for selecting groups of pivot vectors by means of randomized projections. It is demonstrated that the asymptotic flop count for the proposed method is $2mn^2 - (2/3)n^3$ for an $m\times n$ matrix, identical to that of the best classical unblocked Householder QR factorization algorithm (with or without pivoting). Experiments demonstrate acceleration in speed of close to an order of magnitude relative to the {\sc geqp3} function in LAPACK, when executed on a modern CPU with multiple cores. Further, experiments demonstrate that the quality of the randomized pivot selection strategy is roughly the same as that of classical column pivoting. The described algorithm is made available under Open Source license and can be used with LAPACK or libflame.

==> 031cost.tex <==
CONSIDER m x n VERSUS n x n HERE.

In analyzing the cost of the algorithm, we note that all steps in Fig.~\ref{fig:HQRRPblk}
highlighted in grey are part of the blocked HQR
algorithm, which is known to have a cost of approximately $ 4/3 n^3 $ flops.
This leaves us to discuss the overhead related to the other
operations.
\begin{itemize}
\item
{$ G := \mbox{\sc rand\_iid}( b + p, n( A ) )) $:}
Cost: ignored.
\item
{$ Y := G A $:}
Cost: $ 2 ( b + p ) n^2 $ flops.
\item
{$ s_1  := \mbox{\sc DeterminePivots}(
        \FlaOneByTwoSingleLine{ Y_1 }{ Y_2 }, b )  $:}
Cost: $ O( b (b + p ) ( n - kb ) )$ flops
\RvdG{during the $ k $th iteration of the blocked algorithm, for a total of
$ O( (b+p)n^2)$ flops}.  (Recall that the factorization of this matrix
can stop after the first $ b $ columns have been identified.)
%% \item
%% $ \left( \begin{array}{c | c}
%% A_{01} & A_{02} \\ \whline
%% A_{11} & A_{12} \\ \hline
%% A_{21} & A_{22}
%% \end{array} \right)
%% := \mbox{\sc SwapCols}( s_1,
%% \left( \begin{array}{c | c}
%% A_{01} & A_{02} \\ \whline
%% A_{11} & A_{12} \\ \hline
%% A_{21} & A_{22}
%% \end{array} \right)
%% ) $\\
%% Cost: ignored.
\item
{$ \cdots
:=
\mbox{\sc SwapCols}( s_1, \cdots  ) $:}
Cost: ignored.
\item
{$ Y_2
:=
Y_2 -
\left(  G_1
 - ( G_1 U_{11} + G_2 {U_{21}} )
T_{11}^{-1} {U_{11}}^H  \right) { R_{12} } $:}
Aggregate cost: $ O( (b+p) n^2 ) $.
\end{itemize}
Thus,
the overhead is
$ O( (b+p)  n^2 )$ flops and the total cost is
\[
4/3 n^3
+
O( (b+p)  n^2 )
\mbox{ flops},
\]
which, asymptotically, approaches $  4/3 n^3 $ flops.
An analogous analysis of the cost for factoring a rectangular matrix shows that
the asymptotic flop count is $2 mn^2 - \frac{2}{3} n^3$ whenever $m \geq n$.


==> Graphs/qrp_marbore_1c.tex <==
\begin{figure}[ptb]

\begin{center}
\begin{tikzpicture}
  \begin{axis}[
    title= One core,
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.65\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS},
               xmin=0,xmax=10,ymin=0,ymax=27.853,
               legend style={legend pos=outer north east},
%               legend style={overlay,at={(-0.5,10)},anchor=center},
               clip=true,cycle list name=mark list],
  \addplot coordinates {
    (1,1)
    (2,2)
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \legend{%
    \begin{minipage}{0.25\textwidth}\footnotesize dgeqrf\end{minipage},
    \begin{minipage}{0.25\textwidth}\footnotesize dgeqp3\end{minipage},
    \begin{minipage}{0.25\textwidth}\footnotesize HQRRP\end{minipage},
    \begin{minipage}[t]{0.25\textwidth}\footnotesize HQRRP ($Y$ downdate)\end{minipage},
  }
  \end{axis}
\end{tikzpicture}

\vspace{0.2in}
\begin{tikzpicture}
  \begin{axis}[
    title= Four cores,
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.65\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS per core},
               xmin=0,xmax=10,ymin=0,ymax=27.853,
%               legend style={legend pos=north west},
               legend pos=outer north east,
               clip=true,cycle list name=mark list],
  \addplot coordinates {
    (1,1)
    (2,2)
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \addplot coordinates {
    (2,2) 
    (3,3) 
  };
  \legend{%
    \begin{minipage}{0.25\textwidth}\footnotesize dgeqrf\end{minipage},
    \begin{minipage}{0.25\textwidth}\footnotesize dgeqp3\end{minipage},
    \begin{minipage}{0.25\textwidth}\footnotesize HQRRP\end{minipage},
    \begin{minipage}[t]{0.25\textwidth}\footnotesize HQRRP ($Y$ downdate)\end{minipage},
  }
  \end{axis}
\end{tikzpicture}
\end{center}

\caption{Performance of the various implementations.  The top of each 
  graph represents theoretical peak performance.}
\label{fig:performance}

\end{figure}



==> Graphs/qrp_marbore_graphs.tex <==
\begin{figure}[ptb]

\begin{center}
\begin{tikzpicture}
  \begin{axis}[
    title= One core,
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.65\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS per core},
               xmin=0,xmax=10,ymin=0,ymax=45,
%               legend style={legend pos=north west},
               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
],
% dgeqrf
  \addplot coordinates {
( 500/1000,  14.83 )
( 1000/1000,  26.32 )
( 2000/1000,  30.71 )
( 3000/1000,  31.77 )
( 4000/1000,  31.99 )
( 5000/1000,  33.07 )
( 6000/1000,  33.33 )
( 8000/1000,  34.11 )
( 10000/1000,  34.75 )
  };
% qrrp with downdate
  \addplot coordinates {
( 500/1000,  7.43 )
( 1000/1000,  12.58 )
( 2000/1000,  18.75 )
( 3000/1000,  21.42 )
( 4000/1000,  23.54 )
( 5000/1000,  24.96 )
( 6000/1000,  26.02 )
( 8000/1000,  27.75 )
( 10000/1000,  28.62 )
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
( 500/1000,  10.54 )
( 1000/1000,  15.32 )
( 2000/1000,  20.14 )
( 3000/1000,  21.51 )
( 4000/1000,  22.13 )
( 5000/1000,  23.04 )
( 6000/1000,  23.44 )
( 8000/1000,  24.25 )
( 10000/1000,  21.96 )
  };
% qrrp without downdate
  \addplot coordinates {
( 500/1000,  6.42 )
( 1000/1000,  10.02 )
( 2000/1000,  13.80 )
( 3000/1000,  15.13 )
( 4000/1000,  15.99 )
( 5000/1000,  16.77 )
( 6000/1000,  17.36 )
( 8000/1000,  18.01 )
( 10000/1000,  18.39 )
  };
% geqp3
  \addplot coordinates {
( 500/1000,  6.27 )
( 1000/1000,  7.88 )
( 2000/1000,  8.62 )
( 3000/1000,  5.37 )
( 4000/1000,  4.38 )
( 5000/1000,  4.28 )
( 6000/1000,  4.23 )
( 8000/1000,  4.08 )
( 10000/1000,  4.12 )
  };
  \legend{%
    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRPddY\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
  }
  \end{axis}
\end{tikzpicture}

\vspace{0.2in}
\begin{tikzpicture}
  \begin{axis}[
    title= Four cores,
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.65\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS per core},
               xmin=0,xmax=10,ymin=0,ymax=30,
%               legend style={legend pos=north west},
               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
% dgeqrf
  \addplot coordinates {
(  500/1000,    8.57/4 )
(  1000/1000,   30.72/4 )
( 2000/1000,   43.53/4 )
( 3000/1000,   51.01/4 )
( 4000/1000,   52.85/4 )
( 5000/1000,   57.43/4 )
( 6000/1000,   58.83/4 )
( 8000/1000,   60.47/4 )
( 10000/1000,   62.98/4 )
  };
% qrrp with downdate
  \addplot coordinates {
( 500/1000,    6.39/4 )
( 1000/1000,   12.52/4 )
( 2000/1000,   22.25/4 )
( 3000/1000,   27.28/4 )
( 4000/1000,   31.64/4 )
( 5000/1000,   36.19/4 )
( 6000/1000,   39.08/4 )
( 8000/1000,   43.61/4 )
( 10000/1000,   46.69/4 )
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
( 500/1000,    9.93/4 )
( 1000/1000,   16.45/4 )
( 2000/1000,   23.75/4 )
( 3000/1000,   27.01/4 )
( 4000/1000,   28.79/4 )
( 5000/1000,   30.49/4 )
( 6000/1000,   32.43/4 )
( 8000/1000,   33.61/4 )
( 10000/1000,   28.64/4 )
  };
% qrrp without downdate
  \addplot coordinates {
( 500/1000,    5.21/4 )
( 1000/1000,    9.58/4 )
( 2000/1000,   16.01/4 )
( 3000/1000,   18.95/4 )
( 4000/1000,   21.45/4 )
( 5000/1000,   24.22/4 )
( 6000/1000,   25.82/4 )
( 8000/1000,   28.17/4 )
( 10000/1000,   29.76/4 )
  };
% geqp3
  \addplot coordinates {
( 500/1000,    8.52/4 )
( 1000/1000,   12.22/4 )
( 2000/1000,   15.16/4 )
( 3000/1000,    9.10/4 )
( 4000/1000,    6.95/4 )
( 5000/1000,    6.72/4 )
( 6000/1000,    6.50/4 )
( 8000/1000,    6.55/4 )
( 10000/1000,    6.55/4 )
  };
  \legend{%
    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRPddY\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
  }
  \end{axis}
\end{tikzpicture}
\end{center}

\caption{Performance of the various implementations.  The top of each 
  graph represents theoretical peak performance.}
\label{fig:performance}

\end{figure}



==> Graphs/qrp_marbore_graphs_sidebyside.tex <==
\begin{figure}[ptb]

\begin{center}
\begin{tikzpicture}
  \begin{axis}[
    title= {One core $ b=64$},
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.495\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS},
               xmin=0,xmax=10,ymin=0,ymax=40,
%               legend style={legend pos=north west},
%               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
],
% dgeqrf
  \addplot coordinates {
( 500/1000,  14.83 )
( 1000/1000,  26.32 )
( 2000/1000,  30.71 )
( 3000/1000,  31.77 )
( 4000/1000,  31.99 )
( 5000/1000,  33.07 )
( 6000/1000,  33.33 )
( 8000/1000,  34.11 )
( 10000/1000,  34.75 )
  };
% qrrp with downdate
  \addplot coordinates {
( 500/1000,  7.43 )
( 1000/1000,  12.58 )
( 2000/1000,  18.75 )
( 3000/1000,  21.42 )
( 4000/1000,  23.54 )
( 5000/1000,  24.96 )
( 6000/1000,  26.02 )
( 8000/1000,  27.75 )
( 10000/1000,  28.62 )
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
( 500/1000,  10.54 )
( 1000/1000,  15.32 )
( 2000/1000,  20.14 )
( 3000/1000,  21.51 )
( 4000/1000,  22.13 )
( 5000/1000,  23.04 )
( 6000/1000,  23.44 )
( 8000/1000,  24.25 )
( 10000/1000,  21.96 )
  };
% qrrp without downdate
  \addplot coordinates {
( 500/1000,  6.42 )
( 1000/1000,  10.02 )
( 2000/1000,  13.80 )
( 3000/1000,  15.13 )
( 4000/1000,  15.99 )
( 5000/1000,  16.77 )
( 6000/1000,  17.36 )
( 8000/1000,  18.01 )
( 10000/1000,  18.39 )
  };
% geqp3
  \addplot coordinates {
( 500/1000,  6.27 )
( 1000/1000,  7.88 )
( 2000/1000,  8.62 )
( 3000/1000,  5.37 )
( 4000/1000,  4.38 )
( 5000/1000,  4.28 )
( 6000/1000,  4.23 )
( 8000/1000,  4.08 )
( 10000/1000,  4.12 )
  };
%%%  \legend{%
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt HQRRPddY\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
%%%  }
  \end{axis}
\end{tikzpicture}
\begin{tikzpicture}
  \begin{axis}[
    title= {Four cores $ b=64$},
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.495\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS per core},
               xmin=0,xmax=10,ymin=0,ymax=40,
               legend style={legend pos=north east},
%               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
% dgeqrf
  \addplot coordinates {
(  500/1000,    8.57/4 )
(  1000/1000,   30.72/4 )
( 2000/1000,   43.53/4 )
( 3000/1000,   51.01/4 )
( 4000/1000,   52.85/4 )
( 5000/1000,   57.43/4 )
( 6000/1000,   58.83/4 )
( 8000/1000,   60.47/4 )
( 10000/1000,   62.98/4 )
  };
% qrrp with downdate
  \addplot coordinates {
( 500/1000,    6.39/4 )
( 1000/1000,   12.52/4 )
( 2000/1000,   22.25/4 )
( 3000/1000,   27.28/4 )
( 4000/1000,   31.64/4 )
( 5000/1000,   36.19/4 )
( 6000/1000,   39.08/4 )
( 8000/1000,   43.61/4 )
( 10000/1000,   46.69/4 )
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
( 500/1000,    9.93/4 )
( 1000/1000,   16.45/4 )
( 2000/1000,   23.75/4 )
( 3000/1000,   27.01/4 )
( 4000/1000,   28.79/4 )
( 5000/1000,   30.49/4 )
( 6000/1000,   32.43/4 )
( 8000/1000,   33.61/4 )
( 10000/1000,   28.64/4 )
  };
% qrrp without downdate
  \addplot coordinates {
( 500/1000,    5.21/4 )
( 1000/1000,    9.58/4 )
( 2000/1000,   16.01/4 )
( 3000/1000,   18.95/4 )
( 4000/1000,   21.45/4 )
( 5000/1000,   24.22/4 )
( 6000/1000,   25.82/4 )
( 8000/1000,   28.17/4 )
( 10000/1000,   29.76/4 )
  };
% geqp3
  \addplot coordinates {
( 500/1000,    8.52/4 )
( 1000/1000,   12.22/4 )
( 2000/1000,   15.16/4 )
( 3000/1000,    9.10/4 )
( 4000/1000,    6.95/4 )
( 5000/1000,    6.72/4 )
( 6000/1000,    6.50/4 )
( 8000/1000,    6.55/4 )
( 10000/1000,    6.55/4 )
  };
  \legend{%
    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRPbasic\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
  }
  \end{axis}
\end{tikzpicture}
\\
\begin{tikzpicture}
  \begin{axis}[
    title= {One core $ b=128$},
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.495\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS},
               xmin=0,xmax=10,ymin=0,ymax=40,
%               legend style={legend pos=north west},
%               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
],
% dgeqrf
  \addplot coordinates {
(  500/1000,  11.36)
(  1000/1000,  21.48)
(  2000/1000,  27.47)
(  3000/1000,  30.39)
(  4000/1000,  31.72)
(  5000/1000,  33.40)
(  6000/1000,  34.31)
(  8000/1000,  35.70)
( 10000/1000,  36.79)
  };
% qrrp with downdate
  \addplot coordinates {
(  500/1000,   5.06)
(  1000/1000,   9.22)
(  2000/1000,  15.08)
(  3000/1000,  19.03)
(  4000/1000,  21.61)
(  5000/1000,  23.84)
(  6000/1000,  25.47)
(  8000/1000,  28.28)
( 10000/1000,  30.09)
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
(  500/1000,   8.32)
(  1000/1000,  13.26)
(  2000/1000,  18.42)
(  3000/1000,  20.58)
(  4000/1000,  21.55)
(  5000/1000,  23.09)
(  6000/1000,  23.72)
(  8000/1000,  24.29)
( 10000/1000,  21.24)
  };
% qrrp without downdate
  \addplot coordinates {
(  500/1000,   5.14)
(  1000/1000,   8.53)
(  2000/1000,  12.86)
(  3000/1000,  14.95)
(  4000/1000,  16.55)
(  5000/1000,  17.79)
(  6000/1000,  18.65)
(  8000/1000,  19.71)
( 10000/1000,  20.49)
  };
% geqp3
  \addplot coordinates {
(  500/1000,   6.04)
(  1000/1000,   7.68)
(  2000/1000,   8.46)
(  3000/1000,   5.33)
(  4000/1000,   4.36)
(  5000/1000,   4.26)
(  6000/1000,   4.20)
(  8000/1000,   4.07)
( 10000/1000,   4.11)
  };
%%%  \legend{%
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt HQRRPddY\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
%%%    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
%%%  }
  \end{axis}
\end{tikzpicture}
\begin{tikzpicture}
  \begin{axis}[
    title= {Four cores $ b=128$},
               xtick={%
%                 1,
                 2,
%                 3,
                 4,
%                 5,
                 6,
%                 7,
                 8,
%                 9,
                 10},
               xticklabels={%
%                 \mbox{\begin{sideways}1000\end{sideways}},
                 \mbox{\begin{sideways}2000\end{sideways}},
%                 \mbox{\begin{sideways}3000\end{sideways}},
                 \mbox{\begin{sideways}4000\end{sideways}},
%                 \mbox{\begin{sideways}5000\end{sideways}},
                 \mbox{\begin{sideways}6000\end{sideways}},
%                 \mbox{ \begin{sideways}7000\end{sideways}},
                 \mbox{ \begin{sideways}8000\end{sideways}},
%                 \mbox{ \begin{sideways}9000\end{sideways}},
                 \mbox{ \begin{sideways}10000\end{sideways}}
               },
               xmajorgrids,ymajorgrids,
               width=0.495\textwidth,
               height=0.5\textwidth,
               xlabel=\mbox{$m =n$},
               ylabel={GFLOPS per core},
               xmin=0,xmax=10,ymin=0,ymax=40,
               legend style={legend pos=north east},
%               legend pos=outer north east,
               clip=true],
%,cycle list name=mark list],
% dgeqrf
  \addplot coordinates {
(  500/1000,  7.04/4 )
( 1000/1000,  23.18/4 )
( 2000/1000,  36.11/4 )
( 3000/1000,  43.11/4 )
( 4000/1000,  48.72/4 )
( 5000/1000,  52.59/4 )
( 6000/1000,  54.04/4 )
( 8000/1000,  58.36/4 )
( 10000/1000, 60.80/4 )
  };
% qrrp with downdate
  \addplot coordinates {
( 500 /1000,   4.14/4 )
( 1000/1000,   8.91/4 )
( 2000/1000,  16.44/4 )
( 3000/1000,  22.21/4 )
( 4000/1000,  27.68/4 )
( 5000/1000,  31.13/4 )
( 6000/1000,  34.62/4 )
( 8000/1000,  40.20/4 )
( 10000/1000, 43.62/4 )
  };
% dgeqpx (window pivoting)
  \addplot coordinates {
( 500 /1000,   7.60/4 )
( 1000/1000,  13.41/4 )
( 2000/1000,  20.40/4 )
( 3000/1000,  24.35/4 )
( 4000/1000,  27.27/4 )
( 5000/1000,  29.25/4 )
( 6000/1000,  30.49/4 )
( 8000/1000,  31.72/4 )
( 10000/1000, 25.47/4 )
  };
% qrrp without downdate
  \addplot coordinates {
( 500 /1000,   3.83/4 )
( 1000/1000,   7.84/4 )
( 2000/1000,  13.56/4 )
( 3000/1000,  17.38/4 )
( 4000/1000,  21.14/4 )
( 5000/1000,  23.67/4 )
( 6000/1000,  25.41/4 )
( 8000/1000,  28.83/4 )
( 10000/1000, 30.51/4 )
  };
% geqp3
  \addplot coordinates {
( 500 /1000,   6.92/4 )
( 1000/1000,  11.80/4 )
( 2000/1000,  14.70/4 )
( 3000/1000,   9.00/4 )
( 4000/1000,   7.05/4 )
( 5000/1000,   6.69/4 )
( 6000/1000,   6.45/4 )
( 8000/1000,   6.61/4 )
( 10000/1000,  6.48/4 )
  };
  \legend{%
    \begin{minipage}{0.5in}\footnotesize \tt dgeqrf\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRP\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqpx\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt HQRRPbasic\end{minipage},
    \begin{minipage}{0.5in}\footnotesize \tt dgeqp3\end{minipage},
  }
  \end{axis}
\end{tikzpicture}
\end{center}

\caption{Performance of the various implementations.  There is a substantial
  degradation in performance from one core to four.  However, what is
  important is that the relative performance of the different
  algorithms remains essentially the same. This pattern continues as
  more cores are added, as shown in Figure \ref{fig:speedup}.}
\label{fig:performance}

\end{figure}



==> HQRFormTunbvar2.tex <==

\resetsteps      % Reset all the commands to create a blank worksheet  

% Define the operation to be computed

\renewcommand{\routinename}{ \left[ A, T \right] := \mbox{\sc HouseQR\_and\_FormT\_unb\_var2}( A, T ) }

% Step 3: Loop-guard 

\renewcommand{\guard}{
  m( A_{TL} ) < m( A )
}

% Step 4: Define Initialize 

\renewcommand{\partitionings}{
  $
  A \rightarrow
  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  $
,
  $
  T \rightarrow
  \FlaTwoByTwo{T_{TL}}{T_{TR}}
              {T_{BL}}{T_{BR}}
  $
}

\renewcommand{\partitionsizes}{
$ A_{TL} $ is $ 0 \times 0 $,
$ T_{TL} $ is $ 0 \times 0 $
}

% Step 5a: Repartition the operands 

\renewcommand{\repartitionings}{
$  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{A_{00}}{a_{01}}{A_{02}}
                    {a_{10}^T}{\alpha_{11}}{a_{12}^T}
                    {A_{20}}{a_{21}}{A_{22}}
$,
$  \FlaTwoByTwo{T_{TL}}{T_{TR}}
              {T_{BL}}{T_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{T_{00}}{t_{01}}{T_{02}}
                    {0}{\tau_{11}}{t_{12}^T}
                    {0}{0}{T_{22}}
$}

\renewcommand{\repartitionsizes}{
  $ \alpha_{11} $ is $ 1 \times 1 $,
  $ \tau_{11} $ is $ 1 \times 1 $}

% Step 5b: Move the double lines 

\renewcommand{\moveboundaries}{
$  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{A_{00}}{a_{01}}{A_{02}}
                    {a_{10}^T}{\alpha_{11}}{a_{12}^T}
                    {A_{20}}{a_{21}}{A_{22}}
$,
$  \FlaTwoByTwo{T_{TL}}{T_{TR}}
              {T_{BL}}{T_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{T_{00}}{t_{01}}{T_{02}}
                    {0}{\tau_{11}}{t_{12}^T}
                    {0}{0}{T_{22}}
$}

% Step 8: Insert the updates required to change the 
%         state from that given in Step 6 to that given in Step 7
% Note: The below needs editing!!!

\renewcommand{\update}{
$
\begin{array}{l}
\FlaThreeByOneB
{a_{01}} 
{\alpha_{11}}
{a_{02}}
\becomes
\left( 
I
-
\FlaThreeByOneB
  { U_{00} }
  { u_{10}^T }
  { U_{20} } 
T_{00}^{-1}
\FlaThreeByOneB
  { U_{00} }
  { u_{10}^T }
  { U_{20} }^H
\right)^H
\FlaThreeByOneB
  { a_{01} }
  { \alpha_{11} }
  { a_{21} }
\\
\mbox{\ \hspace{0.2in}
\begin{minipage}{4in}
via the steps 
\begin{itemize}
\item
$ w_{01} \becomes T_{00}^{-H} ( U_{00}^H a_{01} + \alpha_{11} ( u_{10}^T )^H +
U_{20}^H a_{21} )  $
\item
$ 
\FlaThreeByOneB
{a_{01}} 
{\alpha_{11}}
{a_{02}}
\becomes
\FlaThreeByOneB
{a_{01}} 
{\alpha_{11}}
{a_{02}}
-
\FlaThreeByOneB
  { U_{00} }
  { u_{10}^T }
  { U_{20} } 
w_{01}
$
\end{itemize}
\end{minipage}
}
\\
\left[
\FlaTwoByOneSingleLine
{ \alpha_{11} }
{ a_{21}}, \tau_{11}
\right]
\becomes
%%% \left[
%%% \FlaTwoByOneSingleLine
%%% { \rho_{11} }
%%% { u_{21}}, \tau_{11}
%%% \right]
%%% =
\housev
\left( \begin{array}{c}
\alpha_{11} \\ \hline
a_{21}
\end{array}
\right) 
\\
t_{01} := ( a_{10}^T )^H + A_{20}^H a_{21}
\end{array}
$ 
}


\begin{figure}[tbp]
%%% \begin{algorithm}
%%% $\left[ A, t \right] \becomes \URt( A )$
%%% \end{algorithm}
% \footnotesize
\FlaAlgorithm
\caption{Alternative unblocked Householder transformation based QR factorization
  merged with the computation of $ T $ for the UT transform.}
\label{fig:HQRFormTunbvar2}
\end{figure}


==> HQRRP_unb_blk.tex <==
\begin{figure}[tb!]

\begin{tabular}{p{0.47\textwidth} c}
\begin{minipage}{3in}
\input RRQR_unb_var3
\FlaAlgorithmNarrow
\end{minipage}
&
\begin{minipage}{3in}
\input RRQR_blk
\FlaAlgorithmNarrow
\end{minipage}
\end{tabular}
\caption{
Left: Unblocked HQRP.
Right: Blocked HQRP.
}
\label{fig:HQRP_unb_blk}
\end{figure}


==> HQRblk.tex <==

\resetsteps      % Reset all the commands to create a blank worksheet  

% Define the operation to be computed

\renewcommand{\routinename}{ \left[ A, t \right] := \mbox{\sc HQR\_blk\_var1}( A, t ) }

% Step 3: Loop-guard 

\renewcommand{\guard}{
  m( A_{TL} ) < m( A )
}

% Step 4: Define Initialize 

\renewcommand{\partitionings}{
  $
  A \rightarrow
  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  $
,
\\
~~~
  $
  t \rightarrow
  \FlaTwoByOne{t_{T}}
              {t_{B}}
  $
}

\renewcommand{\partitionsizes}{
$ A_{TL} $ is $ 0 \times 0 $,
$ t_{T} $ has $ 0 $ rows
}

% Step 5a: Repartition the operands 

\renewcommand{\blocksize}{b}

\renewcommand{\repartitionings}{
$  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  \rightarrow
  \FlaThreeByThreeBR{A_{00}}{A_{01}}{A_{02}}
                    {A_{10}}{A_{11}}{A_{12}}
                    {A_{20}}{A_{21}}{A_{22}}
$,
\\
$  \FlaTwoByOne{ t_T }
              { t_B }
\rightarrow
  \FlaThreeByOneB{t_0}
                 {t_1}
                 {t_2}
$
}

\renewcommand{\repartitionsizes}{
  $ A_{11} $ is $ b \times b $,
  $ t_1 $ has $ b $ rows}

% Step 5b: Move the double lines 

\renewcommand{\moveboundaries}{
$  \FlaTwoByTwo{A_{TL}}{A_{TR}}
              {A_{BL}}{A_{BR}}
  \leftarrow
  \FlaThreeByThreeTL{A_{00}}{A_{01}}{A_{02}}
                    {A_{10}}{A_{11}}{A_{12}}
                    {A_{20}}{A_{21}}{A_{22}}
$,
\\
$  \FlaTwoByOne{ t_T }
               { t_B }
\leftarrow
  \FlaThreeByOneT{t_0}
                 {t_1}
                 {t_2}
$
}

% Step 8: Insert the updates required to change the 
%         state from that given in Step 6 to that given in Step 7
% Note: The below needs editing!!!

\renewcommand{\update}{
$
  \begin{array}{l}
[
\FlaTwoByOneSingleLine
  { A_{11} }
  { A_{21} }, t_1 ]
:= \mbox{\sc HQR\_unb}( 
\FlaTwoByOneSingleLine
  { A_{11} }
  { A_{21} } ) \\
T_{11} := \mbox{\sc FormT}( 
\FlaTwoByOneSingleLine
  { A_{11} }
  { A_{21} }, t_1 )
\\
W_{12} := 
T_{11}^{-H} ( U_{11}^H A_{12} + U_{21}^H A_{22} ) \\
\FlaTwoByOneSingleLine
  { A_{12} }
  { A_{22} }
:= 
\FlaTwoByOneSingleLine
  { A_{12} - U_{11} W_{12} }
  { A_{22} - U_{21} W_{12} }
\end{array}
$
}


%%% \begin{figure}[tb!]
%%% \FlaAlgorithm
%%% \caption{Blocked Householder transformation based QR factorization.}
%%% \label{fig:HQRblk}
%%% \end{figure}


==> HQRunb.tex <==
\resetsteps

\renewcommand{\routinename}{[ A, t ] = \mbox{\sc HouseQR\_unb}( A )}
\renewcommand{\guard}{n( A_{BR} ) \neq 0}

\renewcommand{\partitionings}{
$
A \rightarrow
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   }
$
and
$
t \rightarrow
\FlaTwoByOne{ t_{T} }
            { t_{B} }
$
}
\renewcommand{\partitionsizes}{
$ A_{TL} $ is $ 0 \times 0 $ and $ t_T $ has $ 0 $ elements}

\renewcommand{\repartitionings}{
$
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   } \rightarrow
\FlaThreeByThreeBR{ A_{00} }{ a_{01} }{ A_{02} }
              { a_{10}^T }{ \alpha_{11} }{ a_{12}^T }
              { A_{20} }{ a_{21} }{ A_{22} }
$,
$
\FlaTwoByOne{ t_{T} }
            { t_{B} } \rightarrow
\FlaThreeByOneB{ t_{0} }
              { \tau_{1} }
              { t_{2} }
$
}
\renewcommand{\repartitionsizes}{
$ \alpha_{11} $ and $ \tau_1 $ are  scalars}

\renewcommand{\moveboundaries}{
$
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   } \leftarrow
\FlaThreeByThreeTL{ A_{00} }{ a_{01} }{ A_{02} }
              { a_{10}^T }{ \alpha_{11} }{ a_{12}^T }
              { A_{20} }{ a_{21} }{ A_{22} }
$
,
$
\FlaTwoByOne{ t_{T} }
            { t_{B} } \leftarrow
\FlaThreeByOneT{ t_{0} }
              { \tau_{1} }
              { t_{2} }
$
}

\renewcommand{\update}{
$
\begin{array}{l}
\left[
\FlaTwoByOneSingleLine
{ \alpha_{11} }
{ a_{21}}, \tau_1
\right]
\becomes
%%% \left[
%%% \FlaTwoByOneSingleLine
%%% { \rho_{11} }
%%% { u_{21}}, \tau_1
%%% \right]
%%% =
\housev
\left( \begin{array}{c}
\alpha_{11} \\ \hline
a_{21}
\end{array}
\right) \\
w_{12}^T \becomes ( a_{12}^T + a_{21}^H A_{22} )/\tau_1 \\
\FlaTwoByOneSingleLine
{ a_{12}^T }
{ A_{22} }
\becomes 
\FlaTwoByOneSingleLine
{ a_{12}^T - { w_{12}^T } }
{ A_{22} - { a_{21} } { w_{12}^T } }
\end{array}
$
}

\begin{figure}[tb!]
%%% \begin{algorithm}
%%% $\left[ A, t \right] \becomes \URt( A )$
%%% \end{algorithm}
% \footnotesize
\FlaAlgorithm
\caption{Unblocked Householder transformation based QR factorization.}
\label{fig:HQRunb}
\end{figure}


==> RRQB_unb_var1.tex <==

\resetsteps      % Reset all the commands to create a blank worksheet  

% Define the operation to be computed

\renewcommand{\routinename}{ \left[ A, Q, B \right] := \mbox{\sc RRQB\_blk\_var1}( A, Q, B, k ) }

% Step 3: Loop-guard 

\renewcommand{\guard}{
  n( Q_L ) < k
}

% Step 4: Define Initialize 

\renewcommand{\partitionings}{
  $
  Q \rightarrow
  \FlaOneByTwo{Q_L}{Q_R}
  $
,
  $
  B \rightarrow
  \FlaTwoByOne{B_{T}}
              {B_{B}}
  $
}

\renewcommand{\partitionsizes}{
$ Q_L $ has $ 0 $ columns,
$ B_{T} $ has $ 0 $ rows
}

% Step 5a: Repartition the operands 

\renewcommand{\blocksize}{b}

\renewcommand{\repartitionings}{
$  \FlaOneByTwo{Q_L}{Q_R}
\rightarrow  \FlaOneByThreeR{Q_0}{Q_1}{Q_2}
$
,
$  \FlaTwoByOne{ B_T }
              { B_B }
\rightarrow
  \FlaThreeByOneB{B_0}
                 {B_1}
                 {B_2}
$
}

\renewcommand{\repartitionsizes}{
  $ Q_1 $ has $b$ columns,
  $ B_1 $ has $ b $ rows}

% Step 5b: Move the double lines 

\renewcommand{\moveboundaries}{
$  \FlaOneByTwo{Q_L}{Q_R}
\leftarrow  \FlaOneByThreeL{Q_0}{Q_1}{Q_2}
$
,
$  \FlaTwoByOne{ B_T }
               { B_B }
\leftarrow
  \FlaThreeByOneT{B_0}
                 {B_1}
                 {B_2}
$
}

% Step 8: Insert the updates required to change the 
%         state from that given in Step 6 to that given in Step 7
% Note: The below needs editing!!!

\renewcommand{\update}{
$
  \begin{array}{l @{\hspace{0.5in}} l}
& \mbox{flops} \\ 
U = {\rm rand}( n( A ), b ) \\
A U \rightarrow Q_1 R & 2 m n b + 2 m b^2 - \frac{2}{3} b^3 \\
B_1 = Q_1^T A & 2 m n b \\
A = A - Q_1 B_1 & 2 m n b 
  \end{array}
$
}

\begin{figure}[tb!]
\FlaAlgorithm
\caption{Blocked Householder transformation based QR factorization with column pivoting based on randomization.}
\label{fig:HQRblk}
\end{figure}




==> RRQR.tex <==
This section is under construction.

It may be good at this point to skip forward to 
Section~\ref{sec:PermutationMatrices} and learn about permutation matrices. 

\subsection{Motivation}

Given $ A \in \mathbb{C}^{m \times n} $, with $ m \geq n $, the reduced QR
factorization $ A = Q R $ yields $ Q \in \mathbb{C}^{m \times n} $,
the columns of which form an orthonormal basis for the column space of
$ A $. 
If the matrix has rank $ r $ with $ r < n $, things get a bit
more complicated.   Let $ P $ be a permutation matrix so that the
first $ r $ columns of $ A P^T $ are linearly independent.
Specifically, if we partition
\[
A P^T \rightarrow \FlaOneByTwo{ A_L }{ A_R} ,
\]
where $ A_L $ has $ r $
columns, we can find an orthonormal basis for the column space of $
A_L $ by computing its QR factorization $ A_L = Q_L R_{TL} $, after
which 
\[
A P^T = Q_L \FlaOneByTwo{ R_{TL}}{ R_{TR}}, 
\]
where $ R_{TR} = Q_L^H A_R $.

Now, if $ A $ is merely almost of rank $ r $ (in other words, $ A =
B + E $ where $ B $ has rank $ r $ and $ \| E
\|_2 $ is small), then 
\[
 A P^T = \FlaOneByTwo{ A_L }{ A_R} = 
\FlaOneByTwo{ Q_L }{ Q_R} \FlaTwoByTwo{ R_{TL}}{ R_{TR}}{ 0 }{ R_{BR}
}\approx 
Q_L \FlaOneByTwo{ R_{TL}}{ R_{TR}},
\]
where $ \| R_{BR} \|_2 $ is small.  This is known as the {\em rank revealing
  QR factorization (RRQR)} and it yields a rank $ r $ approximation to
$ A $ given by 
\[
A \approx Q_L \FlaOneByTwo{ R_{TL}}{ R_{TR}}.
\]
The magnitudes of the diagonal elements of $ R $ are typically
chosen to be in decreasing order and some criteria is used to declare
the matrix of rank $ r $, at which point $ R_{BR} $ can be set to
zero.
Computing the RRQR is commonly called the QR factorization with column
pivoting (QRP), for reason that will become apparent.

\subsection{Modifying MGS to Compute QRP}


We are going to give a modification of the MGS  algorithm for computing QRP and then
explain why it works.  
Let us call this the MGS algorithm with column pivoting (MGSP).
In the below discussion, $ p $ is a vector of integers that will
indicate how columns must be swapped in the course of the computation.
\begin{itemize}
\item
Partition
\[
A \rightarrow \FlaOneByTwoSingleLine{ a_1 }{ A_2 }
,
Q \rightarrow \FlaOneByTwoSingleLine{ q_1 }{ Q_2 },
R \rightarrow 
\FlaTwoByTwoSingleLine
  { \rho_{11} }{ r_{12}^T }
  { 0 }{ R_{22} },
p \rightarrow \FlaTwoByOneSingleLine{ \pi_1 }{ p_2 }
\]
\item
Determine the index $ \pi_1 $ of the column of $ \FlaOneByTwoSingleLine{ a_1 }{ A_2 } $ that is
longest.
\item
Permute $  \FlaOneByTwoSingleLine{ a_1 }{ A_2 } :=
\FlaOneByTwoSingleLine{ a_1 }{ A_2 } P( \pi_1 )^T $, swapping column $ a_1 $ with
the column that is longest.  
\item
Compute $ \rho_{11} := \| a_1 \|_2 $.
\item
$ q_1 := a_1 /\rho_{11} $.
\item
Compute $ r_{12}^T := q_1^T A_2 $.  
\item
Update $ A_2 := A_2 - q_1 r_{12}^T $.
\item
Continue the process with the updated matrix $ A_2 $.
\end{itemize}
The elements on the diagonal of $ R $ will be in non-increasing order (and
positive) because updating $ A_2 := A_2 - q_1 r_{12}^T $ inherently
does not increase the length of the columns of $ A_2 $.  After all, the
component in the direction of $ q_1 $ is being subtracted from each
column of $ A_2 $, leaving the component orthogonal to $ q_1 $.

\newcommand{\EXHQRSixSeventeen}{
Let 
$ A = \left( \begin{array}{c | c | c | c}
a_0 & a_1 & \cdots & a_{n-1}
\end{array}
\right) 
$,
$ v = 
\left( \begin{array}{c}
\nu_0 \\
\nu_1 \\
\vdots \\
\nu_{n-1}
\end{array}
\right) 
=
\left( \begin{array}{c}
\| a_0 \|_2^2 \\
\| a_1 \|_2^2 \\
\vdots \\
\| a_{n-1}^2 \|_2 
\end{array}
\right) 
$, 
$ q^T q = 1 $ (of same size as the columns of $ A $), and $ r = A^T
q = 
\left( \begin{array}{c}
\rho_0 \\
\rho_1 \\
\vdots \\
\rho_{n-1}
\end{array} \right)
$.
Compute $ B := A - q r^T $ with 
$ B = \left( \begin{array}{c | c | c | c}
b_0 & b_1 & \cdots & b_{n-1}
\end{array}
\right) 
$.  Then 
\[
\left( \begin{array}{c}
\| b_0 \|_2^2 \\
\| b_1 \|_2^2 \\
\vdots \\
\| b_{n-1} \|_2^2
\end{array}
\right) 
=
\left( \begin{array}{c}
\nu_0 - 
\rho_0^2 \\
\nu_1 - 
\rho_1^2 \\
\vdots \\
\nu_{n-1} - 
\rho_{n-1}^2 
\end{array}
\right).
\]

\Answer{
\[
 a_i =  ( a_i - a_i^T q q ) + a_i^T q q 
\]
 and
\[ (a_i - a_i^T q q )^T q = a_i^T q - a_i^T q q^T q = a_i^T q - a_i^T
q = 0 .
\]   This means that 
\[
 \| a_i \|_2^2 = 
\|  ( a_i - a_i^T q q ) + a_i^T q q \|_2^2 
=
\|  a_i - a_i^T q q \|_2^2  + \| a_i^T q q \|_2^2 
=
\|  a_i - \rho_i q \|_2^2  + \| \rho_i q \|_2^2 
=
\| b_i \|_2^2  + \rho_i^2 
\]
so that
\[
\| b_i \|_2^2  = \| a_i \|_2^2 -  \rho_i^2 = \nu_i - \rho_i^2.
\]
}
}

\EXERCISE{HWHQRSixSeventeen}{\EXHQRSixSeventeen}{AnswerHQRSixSeventeen}

Building on the last exercise, we make an important observation that greatly reduces the cost
of determining the column that is longest.
Let us start by computing $ v $ as the vector such that the $ i $th
entry in $ v $ equals the square of the length of the $ i $th column
of $ A $.
In other words, the $ i $th entry of $ v $ equals the dot product of
the $ i $ column of $ A $ with itself. 
In the above outline for the MGS with column pivoting, we can then
also partition
\[
v \rightarrow \FlaTwoByOneSingleLine
{\nu_1}{v_2}.
\]
The question becomes how $ v_2 $ before the update $ A_2 := A_2 - q_1
r_{12}^T $ compares to $ v_2 $ after that update.  The answer is that
the $ i $th entry of $ v_2 $ must be updated by subtracting off the
square of the $i $th entry of $ r_{12}^T $.  

Let us introduce the functions $ v = \mbox{\sc ComputeWeights}( A ) $ 
and $ v = \mbox{\sc UpdateWeights}{ v, r } $ to compute the described
{\em weight vector} $ v $ and to update a weight vector $ v $ by
subtracting from its elements the squares of the corresponding entries
of $ r $.
Also, the function {\sc DeterminePivot} returns the index of the
largest in the vector, and swaps that entry with the first entry.
A MGS algorithm with column pivoting, {\sc MGSP},  is then given in Figure~\ref{fig:MGSP}.
In that algorithm, $ A $ is overwritten with $ Q $.  

\input HouseQR/MGSP

\subsection{Unblocked Householder QR 
  Factorization with Column Pivoting}

The insights we gained from discussing the {\sc MGSP} algorithm can be
extended to QR factorization algorithms based on Householder
transformations.
The unblocked QR factorization discussed in Section~\ref{sec:HQRunb}
can be supplemented with column pivoting, yielding {\sc HQRP\_unb\_var1} in
Figure~\ref{fig:RRQR_unb_var1}.  

\input HouseQR/RRQR_unb_var1

\subsection{Alternative Unblocked Householder QR 
  Factorization with Column Pivoting}

A moment of reflection tells us that there is no straight forward way
for adding column pivoting to {\sc HQR\_and\_FormT\_unb\_var2}.
The reason is that the remaining columns of $ A $ must be at least
partially updated in order to have enough information to determine how
to permute columns in the next step.  Instead we introduce yet
another variant of HQR that at least partiall overcomes this, and can
also be used in a blocked HQRP algorithm.  Connoisseurs of the LU
factorization will notice it has a bit of a flavor of the Crout
variant for computing that factorization (see Section~\ref{sec:LU:Crout}).

The insights that underlie the blocked QR factorzation discussed in
Section~\ref{sec:QRblocked}
can be summarized by
\[
\begin{array}[t]{c}
\underbrace{
( I - U T^{-T} U^T  )}
\\ 
Q^T  
\end{array}
 \widehat A = R ,
\] 
where $ \widehat A $ represents the orginal contents of $ A $,
$ U $ is the matrix of Householder vectors, $ T $ is computed
from $ U $ as described in Section~\ref{sec:UT}, and $ R $ is upper triangular.

Now, partially into the computation we find ourselves in the state
where
\[
\left(  
I - 
\FlaTwoByOne{ U_{TL} }{U_{BL} } 
T_{TL}^{-H}
\FlaTwoByOne{ U_{TL} }{U_{BL}}^H \right)  
\FlaTwoByTwo 
{ \widehat A_{TL} }{ \widehat A_{TR} }
{ \widehat A_{BL} }{ \widehat A_{BR} }
=
\FlaTwoByTwo 
{ R_{TL} }{ R_{TR} }
{ 0 }{ \widetilde A_{BR} }.  
\] 
The matrix $ A $ at that point contains
\[
\FlaTwoByTwo 
{ U \backslash R_{TL} }{ R_{TR} }
{ U_{BL}  }{ \widetilde A_{BR} }
\] 
by which we mean that the Householder vectors computed so far are
stored below the diagonal of $ R_{TL}$.

Let us manipulate this a bit:
\[
\FlaTwoByTwo 
{ \widehat A_{TL} }{ \widehat A_{TR} }
{ \widehat A_{BL} }{ \widehat A_{BR} }
-
\begin{array}[t]{c}
\underbrace{
\FlaTwoByOne{ U_{TL} }{U_{BL} }
\begin{array}[t]{c}
\underbrace{  
T_{TL}^{-H}
\FlaTwoByOne{ U_{TL} }{U_{BL}}^H 
\FlaTwoByTwo 
{ \widehat A_{TL} }{ \widehat A_{TR} }
{ \widehat A_{BL} }{ \widehat A_{BR} }
} \\
\FlaOneByTwo{ W_{TL} }{W_{TR}}
\end{array}
}
\\
\FlaTwoByTwo  
{ U_{TL} W_{TL} }{ U_{TL} W_{TR} }
{ U_{BL} W_{TL} }{ U_{BL} W_{TR} }
\end{array}
=
\FlaTwoByTwo 
{ R_{TL} }{ R_{TR} }
{ 0 }{ \widetilde A_{BR} }. 
\] 
from which we find that $ \widetilde A_{BR} = \widehat A_{BR} -
U_{BL} W_{TR} $.

Now, what if we do not bother to update $ A_{BR} $ so that instead at
this point in the computation 
$ A $ contains
\[
\FlaTwoByTwo 
{ U \backslash R_{TL} }{ R_{TR} }
{ U_{BL}  }{ \widehat A_{BR} },
\]
but we also have computed and stored $ W_{TR} $.
How would we be able to compute another Householder vector, row of $ R
$, and row of $ W $?

Repartition
\[
\begin{array}[t]{c}
\underbrace{
\FlaTwoByTwo 
{ \widehat A_{TL} }{ \widehat A_{TR} }
{ \widehat A_{BL} }{ \widehat A_{BR} }
-
\FlaTwoByOne{ U_{TL} }{U_{BL} }
\FlaOneByTwo{ W_{TL} }{W_{TR}}
} \\
\FlaThreeByThreeBR
{ \widehat A_{00} }{\widehat a_{01} }{ \widehat A_{02} }
{ \widehat a_{10}^T }{\widehat \alpha_{11} }{ \widehat a_{12}^T }
{ \widehat A_{20} }{\widehat a_{21} }{ \widehat A_{22} }
 -
\FlaThreeByOneB{ U_{00} }{u_{10}^T}{U_{20} }
\FlaOneByThreeR{ W_{00} }{w_{01}}{W_{02} }
\end{array}
=
\begin{array}[t]{c}
\underbrace{
\FlaTwoByTwo 
{ R_{TL} }{ R_{TR} }
{ 0 }{ \widetilde A_{BR} }. 
} \\
\FlaThreeByThreeBR 
{ R_{00} }{ r_{01} }{ R_{02} }
{ 0 }{ \widetilde \alpha_{11} }{ \widetilde a_{12}^T }
{ 0 }{ \widetilde a_{21} }{ \widetilde A_{22} }. 
\end{array}
\]
The important observation is that 
\[
\FlaTwoByTwoSingleLine 
{ \widetilde \alpha_{11} }{ \widetilde a_{12}^T }
{ \widetilde a_{21} }{ \widetilde A_{22} }
=
\FlaTwoByTwoSingleLine 
{ \widehat \alpha_{11} - u_{10}^T w_{01}  }{ \widehat a_{12}^T -
  u_{10}^T W_{02}  }
{ \widehat a_{21}- U_{20} w_{01} }{ \widehat A_{22}- U_{20} W_{02} }
\]

What does this mean?
To update the next rows of $ A $ and $ R $ according to the QR
factorization via Householder transformations
\begin{itemize}
\item 
The contents of $ A $ must be updated by
\begin{itemize}
\item 
$ \alpha_{11} := \alpha_{11} - a_{10}^T w_{01} (= \alpha_{11} -
u_{10}^T w_{01} $). 
\item 
$ a_{21} := a_{21} - A_{20} w_{01} (= a_{21} - U_{20} w_{01} $). 
\item 
$ a_{12}^T := a_{12}^T - a_{10}^T W_{02} (= a_{12}^T - u_{12}^T W_{02} $).
\end{itemize}
This updates those parts of $ A $ consistent with prior computations;
\item
The Householder vector can then be computed, updating $ \alpha_{11} $
and $ a_{12} $;
\item
$ w_{12}^T := a_{12}^T - a_{21}^T A_{22} + ( a_{21}^T  A_{21} ) 
W_{02} ) / \tau 
( = a_{12}^T - u_{21}^T ( A_{22} + U_{21}  
W_{02} ) / \tau 
= a_{12}^T - u_{21}^T  \widetilde A_{22}  / \tau )
$.  This computes the next row of $ W $ (or, more precisely, the part of that
row that will be used in future iterations); and
\item
$ a_{12}^T := a_{12}^T - w_{12}^T $.  This computes the remainder of
the next row of $ R $, overwriting $ A $.
\end{itemize}
The resulting algorithm, 
to which column pivoting is added,  is presented in
Figure~\ref{fig:RRQR_unb_var3}. 
In that figure {\sc HQRP\_unb\_var1} is also given for comparison.  An
extra parameter, $ r $, is added to stop the process after $ r $
columns of $ A $ have been completely computed.  This will allow the
algorithm to be used to compute only the first $ r $ columns of $ Q $
(or rather the Householder vectors from which those columns can be computed) and will also allow it to
be incorporated into a blocked algorithm, as we will discuss next.


\input HouseQR/RRQR_unb_var3 

\subsection{Blocked HQRP}

\input HouseQR/RRQR_blk

Finally, a blocked algorithm that incorporates column pivoting and uses {\sc HQRP\_unb\_var3},
is given in Figure~\ref{fig:RRQR_blk}.  The idea is that the unblocked
algorithm is executed leaving the updating of $ A_{22} $ to happen
periodically, via a matrix-matrix multiplication.  While this casts
some of the computation in terms of matrix-matrix multiplication,
a careful analysis shows that a comparable amount of computation is in
lower performing operations like matrix-vector multiplication.

\subsection{Computing $ Q $}

Given the Householder vectors computed as part of any of the HQRP
algorithms, any number of desired columns of matrix $ Q $ can be
computed using the techniques described in Section~\ref{sec:FormingQ}.

==> RRQR_unb_var1.tex <==
\resetsteps

\renewcommand{\routinename}{[ A, t, p ] = \mbox{\sc
    HQRP\_unb\_var1
}( A )}

\renewcommand{\initialize}{v := ComputeWeights( A )}

\renewcommand{\guard}{n( A_{TL} ) <n( A )}

\renewcommand{\partitionings}{
\footnotesize
$ 
A \rightarrow 
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   }
$
,
$
t \rightarrow 
\FlaTwoByOne{ t_{T} }
            { t_{B} }
$
,
$
p \rightarrow 
\FlaTwoByOne{ p_{T} }
            { p_{B} }
$
,
$
v \rightarrow 
\FlaTwoByOne{ v_{T} }
            { v_{B} }
$
}

\renewcommand{\partitionsizes}{
$ A_{TL} $  is $ 0 \times 0 $  and $ t_T $ has $ 0 $ elements}

\renewcommand{\repartitionings}{
\footnotesize 
$
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   } \rightarrow 
\FlaThreeByThreeBR{ A_{00} }{ a_{01} }{ A_{02} }
              { a_{10}^T }{ \alpha_{11} }{ a_{12}^T }
              { A_{20} }{ a_{21} }{ A_{22} }
$
,
$
\FlaTwoByOne{ t_{T} }
            { t_{B} } \rightarrow 
\FlaThreeByOneB{ t_{0} }
              { \tau_{1} }
              { t_{2} }
$
,
$
\FlaTwoByOne{ p_{T} }
            { p_{B} } \rightarrow 
\FlaThreeByOneB{ p_{0} }
              { \pi_{1} }
              { p_{2} }
$
,
$
\FlaTwoByOne{ v_{T} }
            { v_{B} } \rightarrow 
\FlaThreeByOneB{ v_{0} }
              { \nu_{1} }
              { v_{2} }
$
}
\renewcommand{\repartitionsizes}{
$ \alpha_{11} $ and $ \tau_1 $ are  scalars}

\renewcommand{\moveboundaries}{
\NoShow{
$
\FlaTwoByTwo{ A_{TL} } {A_{TR}}
              { A_{BL} } { A_{BR}   } \leftarrow
\FlaThreeByThreeTL{ A_{00} }{ a_{01} }{ A_{02} }
              { a_{10}^T }{ \alpha_{11} }{ a_{12}^T }
              { A_{20} }{ a_{21} }{ A_{22} }
$
,
$
\FlaTwoByOne{ t_{T} }
            { t_{B} } \leftarrow
\FlaThreeByOneT{ t_{0} }
              { \tau_{1} }
              { t_{2} }
$
}
$ \cdots $
}

\renewcommand{\update}{
$
\begin{array}{l}
[
\left( \begin{array}{c}
\nu_1 \\ \hline 
v_2 
\end{array}
\right),
\pi_1 ] = \mbox{\sc DeterminePivot}( 
\left( \begin{array}{c}
\nu_1 \\ \hline 
v_2 
\end{array}
\right) ) \\
\left( \begin{array}{c | c }
a_{01} & A_{02} \\ \whline 
\alpha_{11} & a_{12}^T \\ \hline 
a_{21} & A_{22} 
\end{array}
\right) 
\becomes 
\left( \begin{array}{c | c}
a_{01} & A_{02} \\ \whline 
\alpha_{11} & a_{12}^T \\ \hline 
a_{21} & A_{22} 
\end{array}
\right) 
P( \pi_1 )^T 
\\
\left[
\FlaTwoByOneSingleLine 
{ \alpha_{11} }
{ a_{21}}, \tau_1 
\right]
\becomes 
\left[
\FlaTwoByOneSingleLine 
{ \rho_{11} }
{ u_{21}}, \tau_1 
\right]
=
\housev 
\left( \begin{array}{c}
\alpha_{11} \\ \hline 
a_{21}
\end{array}
\right) \\
w_{12}^T \becomes ( a_{12}^T + a_{21}^H A_{22} )/\tau_1 \\
\FlaTwoByOneSingleLine 
{ a_{12}^T }
{ A_{22} }
\becomes 
\FlaTwoByOneSingleLine 
{ a_{12}^T - { w_{12}^T } }
{ A_{22} - { a_{21} } { w_{12}^T } }
\\
v_2 = \mbox{\sc UpdateWeight}( v_2, a_{12} ) 
\end{array}
$
}

\begin{figure}[tbp]
%%% \begin{algorithm}
%%% $\left[ A, t \right] \becomes \URt( A )$
%%% \end{algorithm}
% \footnotesize
\FlaAlgorithmWithInit
\caption{Simple unblocked rank revealing QR fractorization via
  Householder transformations (HQRP, unblocked Variant 1).}
\label{fig:RRQR_unb_var1}
\end{figure}


==> flatex.tex <==
\newcolumntype{I}{!{\vrule width 1.5pt}}
\newlength\savedwidth
\newcommand\whline{\noalign{\global\savedwidth\arrayrulewidth
                            \global\arrayrulewidth 1.5pt}%
           \hline
           \noalign{\global\arrayrulewidth\savedwidth}}


% 
% A FLAME algorithm is bracketed by
%
%  \begin{FlameAlg}
%    <statements>
%  \end{FlameAlg}

\newenvironment{FlameAlg}{
\begin{tabbing}
in \= in \= in  \= in  \= in  \= \kill
}
{
\end{tabbing}
}

\newboolean{IsWide}
\setboolean{IsWide}{true}

\newenvironment{FlameAlgNarrow}{
\setboolean{IsWide}{false}
\begin{tabbing}
in \= in \= in  \= in  \= in  \= \kill
}
{
\end{tabbing}
\setboolean{IsWide}{true}
}

%
% A loop in a FLAME algorithm is bracketed by
%
% \FlaDoUntil{ <condition> }
%   Body of the loop
% \FlaEndDo
%
% The body is indented

\newcommand{\FlaDoUntil}[1]{
{ \bf do until #1 } \+ 
}

\newcommand{\FlaDoWhile}[1]{{\bf while #1 do} \+ 
}

% Note: because of the \kill, it is important
% to have a \\ before the \FlaEndDo
% since otherwise the last line before the
% \FlaEndDo will not show

\newcommand{\FlaEndDo}{\- \kill
{\bf endwhile }
}

% In math mode, 
% \FlaTwoByTwo{A}{B}
%             {C}{D}
% creates the picture
%   / A || B \
%   | ==  == |
%   \ C || D /

\newcommand{\FlaTwoByTwo}[4]{
\left( 
\begin{array}{c I c}
#1 & #2 \\ \whline
#3 & #4 
\end{array} 
\right)
}

\newcommand{\FlaTwoByTwoNoPar}[4]{
\begin{array}{c I c}
#1 & #2 \\ \whline
#3 & #4 
\end{array} 
}

\newcommand{\FlaTwoByTwoSingleLineNoPar}[4]{
\begin{array}{c | c}
#1 & #2 \\ \hline
#3 & #4 
\end{array} 
}

\newcommand{\FlaTwoByTwoSingleLine}[4]{
\left(  
\begin{array}{c | c}
#1 & #2 \\ \hline
#3 & #4 
\end{array} 
\right)
}


\newcommand{\FlaTwoByTwoNoLine}[4]{
\left(  
\begin{array}{c  c}
#1 & #2 \\ 
#3 & #4 
\end{array} 
\right)
}

% In math mode, 
% \FlaTwoByOne{A}
%             {C}
% creates the picture
%   / A  \
%   | == |
%   \ C  /

\newcommand{\FlaTwoByOne}[2]{
\left( 
\begin{array}{c}
#1 \\ \whline
#2 
\end{array} 
\right)
}

\newcommand{\FlaTwoByOneNoPar}[2]{
\begin{array}{c}
#1 \\ \whline
#2 
\end{array} 
}

% In math mode, 
% \FlaTwoByOneSingleLine{A}
%                       {C}
% creates the picture
%   / A  \
%   | -- |
%   \ C  /

\newcommand{\FlaTwoByOneSingleLine}[2]{
\left( 
\begin{array}{c}
#1 \\ \hline
#2 
\end{array} 
\right)
}


\newcommand{\FlaTwoByOneNoLine}[2]{
\left( 
\begin{array}{c}
#1 \\
#2 
\end{array} 
\right)
}

% In math mode, 
% \FlaOneByTwo{A}{B}
% creates the picture
%   ( A || B )

\newcommand{\FlaOneByTwo}[2]{
\left( 
\begin{array}{c I c}
#1 & #2 
\end{array} 
\right)
}

\newcommand{\FlaOneByTwoNoPar}[2]{
\begin{array}{c I c}
#1 & #2 
\end{array} 
}

\newcommand{\FlaOneByTwoSingleLine}[2]{
\left( 
\begin{array}{c | c}
#1 & #2
\end{array} 
\right)
}

\newcommand{\FlaOneByTwoNoLine}[2]{
\left( 
\begin{array}{c c}
#1 & #2
\end{array} 
\right)
}

% In math mode, 
% \FlaThreeByThreeTL{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A | B || C \
%   | -- ---  -- |
%   | D | E || F |
%   | ==  ==  == |
%   \ G | H || I /
% Notice: the TL means that the
% center block (E) is part of the
% TL quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeTL}[9]{
\left( 
\begin{array}{c | c I c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \whline
#7 & #8 & #9
\end{array} 
\right) 
}

% In math mode, 
% \FlaThreeByThreeBR{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A || B | C \
%   | ==  ==  == |
%   | D || E | F |
%   | -- ---  -- |
%   \ G || H | I /
% Notice: the BR means that the
% center block (E) is part of the
% BR quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeBR}[9]{
\left( 
\begin{array}{c I c | c}
#1 & #2 & #3 \\ \whline
#4 & #5 & #6 \\ \hline
#7 & #8 & #9
\end{array} 
\right)
}

\newcommand{\FlaThreeByThreeSingleLine}[9]{
\left( 
\begin{array}{c | c | c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \hline
#7 & #8 & #9
\end{array} 
\right)
}

\newcommand{\FlaThreeByThreeNoLine}[9]{
\left( 
\begin{array}{c c c}
#1 & #2 & #3 \\ 
#4 & #5 & #6 \\ 
#7 & #8 & #9
\end{array} 
\right)
}

% In math mode, 
% \FlaThreeByThreeTR{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A || B | C \
%   | -- ---  -- |
%   | D || E | F |
%   | ==  ==  == |
%   \ G || H | I /
% Notice: the TR means that the
% center block (E) is part of the
% TR quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeTR}[9]{
\left( 
\begin{array}{c I c | c}
#1 & #2 & #3 \\ \hline
#4 & #5 & #6 \\ \whline
#7 & #8 & #9
\end{array} 
\right)
}


% In math mode, 
% \FlaThreeByThreeBL{A}{B}{C}
%                   {D}{E}{F}
%                   {G}{H}{I}
% creates the picture
%   / A | B || C \
%   | ==  ==  == |
%   | D | E || F |
%   | -- ---  -- |
%   \ G | H || I /
% Notice: the BL means that the
% center block (E) is part of the
% BL quadrant, where quadrants are
% partitioned by the double lines.

\newcommand{\FlaThreeByThreeBL}[9]{
\left( 
\begin{array}{c | c I c}
#1 & #2 & #3 \\ \whline
#4 & #5 & #6 \\ \hline 
#7 & #8 & #9
\end{array} 
\right)
}

% In math mode, 
% \FlaOneByThreeR{A}{B}{C}
% creates the picture
%   ( A || B | C )
% Notice: the R means that the
% center block (B) is part of the
% R(ight) submatrix, where 
% submatrices are % partitioned 
% by the double lines.

\newcommand{\FlaOneByThreeR}[3]{
\left( 
\begin{array}{c I c | c}
#1 & #2 & #3 
\end{array} 
\right)
}

% In math mode, 
% \FlaOneByThreeL{A}{B}{C}
% creates the picture
%   ( A | B || C )
% Notice: the R means that the
% center block (B) is part of the
% R(ight) submatrix, where 
% submatrices are % partitioned 
% by the double lines.

\newcommand{\FlaOneByThreeL}[3]{
\left( 
\begin{array}{c | c I c}
#1 & #2 & #3 
\end{array} 
\right)
}

% In math mode, 
% \FlaThreeByOneT{A}
%                {D}
%                {G}
% creates the picture
%   / A  \
%   | == |
%   | B  |
%   | -- |
%   \ C  /
% Notice: the T means that the
% center block (C) is part of the
% T(op) submatrix where submatrices
% are % partitioned by the double 
% lines.

\newcommand{\FlaThreeByOneT}[3]{
\left( 
\begin{array}{c}
#1 \\ \hline
#2 \\ \whline
#3 
\end{array} 
\right) 
}

\newcommand{\FlaThreeByOneTNoPar}[3]{
\begin{array}{c}
#1 \\ \hline
#2 \\ \whline
#3 
\end{array} 
}

% In math mode, 
% \FlaThreeByOneB{A}
%                {D}
%                {G}
% creates the picture
%   / A  \
%   | -- |
%   | B  |
%   | == |
%   \ C  /
% Notice: the B means that the
% center block (C) is part of the
% T(op) submatrix where submatrices
% are % partitioned by the double 
% lines.

\newcommand{\FlaThreeByOneB}[3]{
\left( 
\begin{array}{c}
#1 \\ \whline
#2 \\ \hline
#3 
\end{array} 
\right) 
}

\newcommand{\FlaThreeByOneBNoPar}[3]{
\begin{array}{c}
#1 \\ \whline
#2 \\ \hline
#3 
\end{array} 
}

\newcommand{\FlaThreeByOneSingleLine}[3]{
\left( 
\begin{array}{c}
#1 \\ \hline
#2 \\ \hline
#3 
\end{array} 
\right) 
}

\newcommand{\FlaThreeByOneNoLine}[3]{
\left( 
\begin{array}{c}
#1 \\ 
#2 \\ 
#3 
\end{array} 
\right) 
}

% Various key words

% The following is a typical use of 
% \FlaPartition:
% 
% \FlaPartition {
%    $ A \rightarrow \FlaTwoByTwo{ A_{TL} }{ A_{TR} }
%                                { A_{BL} }{ A_{BR} } $ 
% }
% {
%    where $ A_{TL} $ is $ 0 \times 0 $
% }
% 
% Creates something like
% Partition A -> / A_TL || A_TR \
%                | =====  ===== |
%                \ A_BL || A_BR /
% where A_TL is 0 x 0
%

\newcommand{\FlaPartition}[2]{
\ifthenelse{\boolean{IsWide}}{{\bf partition } \hspace{-1em} #1 \hspace{-1em} #2}
{{\bf partition } \+ \\ #1 \+ \\ #2 \- \-}
}

% The following is a typical use of 
% \FlaRepartition:
% 
% \FlaRepartition{
% $ 
% \FlaTwoByTwo{ A_{TL} }{ A_{TR} }
%             { A_{BL} }{ A_{BR} } \rightarrow
% \FlaThreeByThreeBR{ A_{00} }{ A_{01} }{ A_{02} }
%                   { A_{10} }{ A_{11} }{ A_{12} }
%                   { A_{20} }{ A_{21} }{ A_{22} } 
% $ 
% }
% {
%    \FlaWhere{$ A_{11} $ is $ b \times b $}
%  }
% 
% Creates something like
% Repartition  
%   / A_TL || A_TR \    / A_00 || A_01 | A_02 \
%   | =====  ===== | -> | =====  ====== ===== |
%   \ A_BL || A_BR /    | A_10 || A_11 | A_12 |
%                       | -----  ------ ----- |
%                       \ A_20 || A_21 | A_22 /
% where A_11 is b x b
%

\newcommand{\FlaRepartition}[2]{
\ifthenelse{\boolean{IsWide}}{{\bf repartition } \hspace{-1em} #1 \hspace{-1em} #2}
{{\bf repartition } \+ \\ #1 \+ \\ #2 \- \-}
}

% The following is a typical use of 
% \FlaContinue:
% 
% \FlaContinue{
% $ 
%    \FlaTwoByTwo{ A_{TL} }{ A_{TR} }
%                { A_{BL} }{ A_{BR} } \leftarrow
%    \FlaThreeByThreeTL{ A_{00} }{ A_{01} }{ A_{02} }
%                      { A_{10} }{ A_{11} }{ A_{12} }
%                      { A_{20} }{ A_{21} }{ A_{22} } 
% $ 
% }
% 
% Creates something like
% Continue with
%   / A_TL || A_TR \    / A_00 | A_01 || A_02 \
%   | =====  ===== | <- | ----- ------  ----- |
%   \ A_BL || A_BR /    | A_10 | A_11 || A_12 |
%                       | ===== ======  ===== |
%                       \ A_20 | A_21 || A_22 /

\newcommand{\FlaContinue}[1]{
\ifthenelse{\boolean{IsWide}}{{\bf continue with } #1
}
{{\bf continue with } \+ \\ #1 \-
}
}
\newcommand{\FlaWhere}[1]{
\hspace{-1em} { \bf where #1 } 
}

\newcommand{\undetermined}{ \star }

\newcommand{\FlaStartCompute}{%
\setlength{\unitlength}{1.60in}%
\begin{picture}(2,0.01)
\put(0,0){\line(1,0){2}}
\put(0,0.01){\line(1,0){2}}
\end{picture}%
}

\newcommand{\FlaEndCompute}{%
\noindent%
\setlength{\unitlength}{1.60in}%
\begin{picture}(2,0.01)
\put(0,0){\line(1,0){2}} 
\put(0,0.01){\line(1,0){2}} 
\end{picture}%
}

\newcommand{\FlaStartComputeShort}{
\setlength{\unitlength}{1.30in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}}
\put(0,0.01){\line(1,0){3}}
\end{picture} 
}

\newcommand{\FlaEndComputeShort}{
\setlength{\unitlength}{1.30in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}} 
\put(0,0.01){\line(1,0){3}} 
\end{picture} 
}

\newcommand{\FlaStartComputeMedium}{
\setlength{\unitlength}{0.85in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}}
\put(0,0.01){\line(1,0){3}}
\end{picture} 
}

\newcommand{\FlaEndComputeMedium}{
\setlength{\unitlength}{0.85in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}} 
\put(0,0.01){\line(1,0){3}} 
\end{picture} 
}

\newcommand{\FlaStartComputeShorter}{
\setlength{\unitlength}{0.5in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}}
\put(0,0.01){\line(1,0){3}}
\end{picture} 
}

\newcommand{\FlaEndComputeShorter}{
\setlength{\unitlength}{0.5in}
\begin{picture}(3,0.01)
\put(0,0){\line(1,0){3}} 
\put(0,0.01){\line(1,0){3}} 
\end{picture} 
}

\newcommand{\FlaUpLo}[2]{
{#1} \backslash {#2}
}

\newcommand{\FlaInverse}[1]{
{ #1 }^{-1}
}

\newcommand{\Square}{ \mbox{Square} }
\newcommand{\Symm}{ \mbox{Symm} }
\newcommand{\SameSize}{ \mbox{SameSize} }
\newcommand{\RowDim}{\mbox{RowDim}}
\newcommand{\ColDim}{\mbox{ColDim}}
\newcommand{\LowTr}{\mbox{LowTr}}
\newcommand{\UpTr}{\mbox{UpTr}}
\newcommand{\UpperTr}{\mbox{UpTr}}
\newcommand{\UppTr}{\mbox{UpTr}}
\newcommand{\operation}{ [ D, E, F, \ldots ] \becomes {\rm op}( A, B, C, D, \ldots ) }
\newcommand{\routinename}{ [ D, E, F, \ldots ] \becomes {\rm op}( A, B, C, D, \ldots ) }
\newcommand{\routinecost}{ X }
\newcommand{\precondition}{ Q }
\newcommand{\postcondition}{ R }
\newcommand{\invariant}{ P }
\newcommand{\costinv}{ \  }
\newcommand{\costbefore}{ \  }
\newcommand{\costafter}{ \  }
\newcommand{\updatecost}{ \  }
\newcommand{\guard}{ R }
\newcommand{\partitionings}{
\begin{minipage}{3in}
$ S_I $
\end{minipage}
}
\newcommand{\partitionsizes}{ \hspace{ 3.25in} }

\newcommand{\blocksize}{1}

\newcommand{\repartitionings}{
\begin{minipage}[t]{3in}
\ \\
\ \\
\ \\
\end{minipage}
}

\newcommand{\repartitionsizes}{ \hspace{ 3.25in} }
\newcommand{\moveboundaries}{
\begin{minipage}[t]{3in}
\ \\
\ \\
\ \\
\end{minipage}
}
\newcommand{\beforeupdate}{
$ \QBefore $
}
\newcommand{\afterupdate}{
$ \QAfter $
}
\newcommand{\update}{%
\begin{minipage}[t]{4in}
$ S_U $
\end{minipage}
}

\newcommand{\resetsteps}{
\renewcommand{\blocksize}{1}
\renewcommand{\operation}{ [ D, E, F, \ldots ] \becomes {\rm op}( A, B, C, D, \ldots ) }
\renewcommand{\routinename}{ [ D, E, F, \ldots ] \becomes {\rm op}( A, B, C, D, \ldots ) }
\renewcommand{\routinecost}{ 0 }
\renewcommand{\precondition}{ \PPre }
\renewcommand{\postcondition}{ \PPost }
\renewcommand{\invariant}{ \PInv }
\renewcommand{\costinv}{ \  }
\renewcommand{\guard}{ G }
\renewcommand{\partitionings}{ %
\begin{minipage}[t]{3in}
\ \\
\end{minipage}
}
\renewcommand{\partitionsizes}{ \hspace{ 3.25in} }
\renewcommand{\repartitionings}{%
\begin{minipage}[t]{3in}
\ \\
\end{minipage}
}
\renewcommand{\repartitionsizes}{ \hspace{ 3.25in} }
\renewcommand{\moveboundaries}{%
\begin{minipage}[t]{3in}
\ \\
\end{minipage}
}
\renewcommand{\beforeupdate}{
\QBefore
}
\renewcommand{\afterupdate}{
\QAfter
}
\renewcommand{\update}{
$ S_U $
}
}

\newenvironment{FlaBox}{ 
\footnotesize
\begin{framebox}
}
{
\end{framebox}
}

\newcommand{\WSoperation}{ 
$ \operation $
}

\newcommand{\WSprecondition}{
$ \left\{ \precondition \right\} $
}

\newcommand{\WSpostcondition}{
$ \left\{ \postcondition \right\} $
}

\newcommand{\WSinvariant}{
$ \left\{ \invariant \right\} $
}

\newcommand{\WScostinv}{
$ \Csf = \costinv $ flops
}

\newcommand{\WScostzero}{
$ \Csf = 0 $ flops
}

\newcommand{\WScostbu}{
$ \Csf = \costbefore $ flops
}

\newcommand{\WScostau}{
$ \Csf = \costafter $ flops
}

\newcommand{\WSupdatecost}{
{\bf Cost:} $ \updatecost $ flops
}

\newcommand{\WStopofloop}{
$ \left\{ \left( \invariant \right) \wedge \left( \guard \right) \right\} $
}

\newcommand{\WStopofloopnarrow}{
$ \begin{array}{r}
  \left\{ \left( \invariant \right) \right. \\
  \left. \wedge \left( \guard \right) \right\}
\end{array} $
}

\newcommand{\WSafterloop}{
$ \left\{ \left( \invariant \right) \wedge \neg \left( \guard \right) \right\} $
}

\newcommand{\WSguard}{
$ \guard $
}

\newcommand{\WSpartition}{
\begin{minipage}[t]{3in}
\begin{tabbing}
ind \= ind \= \kill
{\bf Partition} 
\partitionings \+ \\
{\bf where } \hspace*{-2ex} \partitionsizes 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSpartitionNarrow}{
\begin{minipage}[t]{2.0in}
\begin{tabbing}
id \= id \= \kill
{\bf Partition} 
\partitionings \+ \\
{\bf where } 
\begin{minipage}[t]{1.5in}
\partitionsizes 
\end{minipage}
\end{tabbing}
\end{minipage}
}

\newcommand{\WSrepartition}{
\begin{minipage}[t]{4.13in}
\ifthenelse{ \equal{\blocksize}{1} }{}
{%
\ifthenelse{ \equal{\blocksize}{blank} }{~}
{{\bf Determine block size $ \blocksize $}} \\
}
{\bf Repartition}
\begin{tabbing}
in \= in \= \+ \kill
\repartitionings \+ \\
{\bf where } \hspace*{-2ex} \repartitionsizes 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSrepartitionMedium}{
\begin{minipage}[t]{2.85in}
\ifthenelse{ \equal{\blocksize}{1} }{}
{%
\ifthenelse{ \equal{\blocksize}{blank} }{~}
{{\bf Determine block size $ \blocksize $}} \\
}
{\bf Repartition}
\begin{tabbing}
in \= in \= \+ \kill
\repartitionings \+ \\
{\bf where } \hspace*{-2ex} \repartitionsizes 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSrepartitionNarrow}{
\begin{minipage}[t]{2.05in}
\ifthenelse{ \equal{\blocksize}{1} }{}
{%
\ifthenelse{ \equal{\blocksize}{blank} }{~}
{{\bf Determine block size $ \blocksize $}} \\
}
{\bf Repartition}
\begin{tabbing}
i \= i \= \+ \kill
\repartitionings \+ \\
{\bf where }
\begin{minipage}[t]{1.5in}
\repartitionsizes
\end{minipage}
\end{tabbing}
\end{minipage}
}

\newcommand{\WSmoveboundary}{
\begin{minipage}[t]{4.13in}
{\bf Continue with}
\begin{tabbing}
ind \= \+ \kill
\moveboundaries 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSmoveboundaryMedium}{
\begin{minipage}[t]{2.85in}
{\bf Continue with}
\begin{tabbing}
ind \= \+ \kill
\moveboundaries 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSmoveboundaryNarrow}{
\begin{minipage}[t]{2.05in}
{\bf Continue with}
\begin{tabbing}
i \= \+ \kill
\moveboundaries 
\end{tabbing}
\end{minipage}
}

\newcommand{\WSbeforeupdate}{
$ \left\{ \beforeupdate \right\} $
}

\newcommand{\WSafterupdate}{
$ \left\{ \afterupdate \right\} $
}

\newcommand{\WSupdate}{
\update
}

\newcommand{\worksheet}{
\begin{center}
\begin{tabular}{| c I l |} \hline
\footnotesize {\bf Step} & 
{\bf Annotated Algorithm:} $\operation$ 
\\ \whline 
\rowcolor[gray]{0.93}
1a & 
\WSprecondition \\ \hline
4 & 
\WSpartition \\ \hline
\rowcolor[gray]{0.93}
2 & 
\WSinvariant \\ \hline
3 & 
{\bf while} \WSguard { \bf do} \\ \hline
\rowcolor[gray]{0.93}
2,3 &
\ \hspace{0.15in} \WStopofloop \\ \hline
5a & 
\ \hspace{0.15in} 
\WSrepartition
\\ \hline
\rowcolor[gray]{0.93}
6 &
\ \hspace{0.15in} \WSbeforeupdate \\ \hline
8 & \ \hspace{0.15in} \WSupdate \\ \hline
5b &
\ \hspace{0.15in} 
\WSmoveboundary
\\ \hline
\rowcolor[gray]{0.93}
7 &
\ \hspace{0.15in} \WSafterupdate \\ \hline 
\rowcolor[gray]{0.93}
2 &
\ \hspace{0.15in} \WSinvariant \\ \hline
& {\bf endwhile} \\ \hline
\rowcolor[gray]{0.93}
2,3 &
\WSafterloop \\ \hline
\rowcolor[gray]{0.93}
1b &
\WSpostcondition \\ \hline
\end{tabular}
\end{center}
}

\newcommand{\worksheetnarrow}{
\begin{center}
\begin{tabular}{| c I l |} \hline
\footnotesize {\bf Step} & 
{\bf Annotated Algorithm:} $\routinename$ 
\\ \whline
\rowcolor[gray]{0.93}
1a & 
\WSprecondition \\ \hline
4 & 
\WSpartition \\ \hline
\rowcolor[gray]{0.93}
2 & 
\WSinvariant \\ \hline
3 & 
{\bf while} \WSguard { \bf do} \\ \hline
\rowcolor[gray]{0.93}
2,3 &
\ \hspace{0.15in} \WStopofloopnarrow \\ \hline
5a & 
\ \hspace{0.15in} 
\WSrepartition
\\ \hline
\rowcolor[gray]{0.93}
6 &
\ \hspace{0.15in} \WSbeforeupdate \\ \hline
8 & \ \hspace{0.15in} \WSupdate \\ \hline
5b &
\ \hspace{0.15in} 
\WSmoveboundary
\\ \hline
\rowcolor[gray]{0.93}
7 &
\ \hspace{0.15in} \WSafterupdate \\ \hline 
\rowcolor[gray]{0.93}
2 &
\ \hspace{0.15in} \WSinvariant \\ \hline
& {\bf endwhile} \\ \hline
\rowcolor[gray]{0.93}
2,3 &
\WSafterloop \\ \hline
\rowcolor[gray]{0.93}
1b &
\WSpostcondition \\ \hline
\end{tabular}
\end{center}
}

\newcommand{\worksheetwithcost}{
\begin{center}
\begin{tabular}{| c I l  r | } \hline
\footnotesize {\bf Step} & 
\multicolumn{2}{l|}
{{\bf Cost Analysis:} $\routinename$} 
\\ \whline
\rowcolor[gray]{0.93}
1a & 
% \WSprecondition 
& \WScostzero \\ \hline
4 & \multicolumn{2}{l|}{
\WSpartition} \\ \hline
\rowcolor[gray]{0.93}
2 & 
% \WSinvariant 
& \WScostinv \\ \hline
3 & \multicolumn{2}{l|}{
{\bf while} \WSguard { \bf do} }\\ \hline
\rowcolor[gray]{0.93}
2,3 &
% \ \hspace{0.15in} \WStopofloop 
& \WScostinv \\ \hline
5a & \multicolumn{2}{l|}{
\ \hspace{0.15in} 
\WSrepartition}
\\ \hline
\rowcolor[gray]{0.93}
6 &
% \ \hspace{0.15in} \WSbeforeupdate
& 
\WScostbu
\\ \hline
8 & 
\hspace{0.15in} \WSupdate
&
\WSupdatecost \\ \hline
5b &\multicolumn{2}{l|}{
\ \hspace{0.15in} 
\WSmoveboundary}
\\ \hline
\rowcolor[gray]{0.93}
7 &
% \ \hspace{0.15in} \WSafterupdate 
& 
\WScostau
\\ \hline 
\rowcolor[gray]{0.93}
2 &
% \ \hspace{0.15in} \WSinvariant
&
\WScostinv \\ \hline
& \multicolumn{2}{l|}{{\bf endwhile}} \\ \hline
\rowcolor[gray]{0.93}
2,3 &
% \WSafterloop
&
\WScostinv
\\ \hline
\rowcolor[gray]{0.93}
1b &
% \WSpostcondition
\multicolumn{2}{r|}
{{\bf Total Cost:} $ \routinecost $ flops}
\\ \hline
\end{tabular}
\end{center}
}

\newcommand{\worksheetnosteps}{
\begin{center}
\begin{tabular}{| l |} \hline
Annotated Algorithm: \WSoperation \\ \whline
\rowcolor[gray]{0.93}
\WSprecondition \\ \hline
\WSpartition \\ \hline
\rowcolor[gray]{0.93}
\WSinvariant \\ \hline
{\bf while} \WSguard { \bf do} \\ \hline
\rowcolor[gray]{0.93}
\ \hspace{0.15in} \WStopofloop \\ \hline
\ \hspace{0.15in} 
\WSrepartition
\\ \hline
\rowcolor[gray]{0.93}
\ \hspace{0.15in} \WSbeforeupdate \\ \hline
\hspace{0.15in} \WSupdate \\ \hline
\ \hspace{0.15in} 
\WSmoveboundary
\\ \hline
\rowcolor[gray]{0.93}
\ \hspace{0.15in} \WSafterupdate \\ \hline 
\rowcolor[gray]{0.93}
\ \hspace{0.15in} \WSinvariant \\ \hline
{\bf endwhile} \\ \hline
\rowcolor[gray]{0.93}
\WSafterloop \\ \hline
\rowcolor[gray]{0.93}
\WSpostcondition \\ \hline
\end{tabular}
\end{center}
}

\newcommand{\worksheetupdate}{
\begin{center}
\begin{tabular}{| c I l |} \hline
\footnotesize Step & Annotated Algorithm: \WSoperation \\ \whline
3 & 
{\bf while} \WSguard { \bf do} \\ \hline
2,3 &
\ \hspace{0.15in} \WStopofloop \\ \hline
5a & 
\ \hspace{0.15in} 
\WSrepartition
\\ \hline
6 &
\ \hspace{0.15in} \WSbeforeupdate \\ \hline
8 & \hspace{0.15in} \WSupdate \\ \hline
5b &
\ \hspace{0.15in} 
\WSmoveboundary
\\ \hline
7 &
\ \hspace{0.15in} \WSafterupdate \\ \hline 
2 &
\ \hspace{0.15in} \WSinvariant \\ \hline
& {\bf endwhile} \\ \hline
\end{tabular}
\end{center}
}

\newcommand{\FlaAlgorithm}{
\begin{center}
\begin{tabular}{|l |} \hline
{\bf Algorithm:} $\routinename$ 
\\ \whline
{\WSpartition} \\[0.3in]
{\bf while} \WSguard { \bf do} \\
\ \hspace{0.15in} \WSrepartition \\
{\hspace{0.15in} \FlaStartComputeShort} \\
{\hspace{0.15in} \WSupdate} \\
{\hspace{0.15in} \FlaEndComputeShort} \\
{\ \hspace{0.15in} \WSmoveboundary} \\
{{\bf endwhile}} \\ \hline
\end{tabular}
\end{center}
}


\newcommand{\FlaAlgorithmMedium}{
\begin{center}
\begin{tabular}{|l |} \hline
{\bf Algorithm:} $\routinename$ 
\\ \whline
{\WSpartition} \\[0.3in]
{\bf while} \WSguard { \bf do} \\
\ \hspace{0.15in} \WSrepartitionMedium \\
{\hspace{0.15in} \FlaStartComputeMedium} \\
{\hspace{0.15in} \WSupdate} \\
{\hspace{0.15in} \FlaEndComputeMedium} \\
{\ \hspace{0.15in} \WSmoveboundaryMedium} \\
{{\bf endwhile}} \\ \hline
\end{tabular}
\end{center}
}


\newcommand{\FlaAlgorithmNarrow}{
\begin{center}
\begin{tabular}{|l |} \hline
{\bf Algorithm:} $\routinename$ 
\\ \whline
{\WSpartitionNarrow} \\
{\bf while} \WSguard { \bf do} \\
\ \hspace{0.0in} \WSrepartitionNarrow \\
{\hspace{0.0in} \FlaStartComputeShorter} \\
{\hspace{0.0in} \WSupdate} \\
{\hspace{0.0in} \FlaEndComputeShorter} \\
{\ \hspace{0.0in} \WSmoveboundaryNarrow} \\
{{\bf endwhile}} \\ \hline
\end{tabular}
\end{center}
}


\newcommand{ \PPre }{ P_{\it pre} }
\newcommand{ \PPost }{ P_{\it post} }
\newcommand{ \PInv }{ P_{\it inv} }
\newcommand{ \PInvone }{ P_{\it inv-1} }
\newcommand{ \PInvtwo }{ P_{\it inv-2} }
\newcommand{ \becomes }{:=}
\newcommand{ \QBefore }{ P_{\it before} }
\newcommand{ \QAfter }{ P_{\it after} }
\newcommand{ \Qbefore }{ P_{\it before} }
\newcommand{ \Qafter }{ P_{\it after} }
\newcommand{ \PCons }{ P_{\it cons} }
\newcommand{ \PCost }{ P_{\it cost} }
\newcommand{ \PStr }{ P_{\it struct} }
\newcommand{ \Csf }{ C_{\it sf} }



==> flatex2_color.tex <==
\newcommand{\FlaComputeSection}[1]{
\color{red}
\setlength{\unitlength}{#1}
\begin{picture}(1,0.01)
\put(0,0){\line(1,0){1}}
\put(0,0.01){\line(1,0){1}}
\end{picture}
}

\newcommand{\routinenameL}{}
\newcommand{\routinenameR}{}

\newcommand{\partitioningsL}{}
\newcommand{\partitioningsR}{}

\newcommand{\partitionsizesL}{}
\newcommand{\partitionsizesR}{}

\newcommand{\repartitioningsL}{}
\newcommand{\repartitioningsR}{}

\newcommand{\repartitionsizesL}{}
\newcommand{\repartitionsizesR}{}

\newcommand{\blocksizeL}{}
\newcommand{\blocksizeR}{}

\newcommand{\moveboundariesL}{}
\newcommand{\moveboundariesR}{}

\newcommand{\updateL}{}
\newcommand{\updateR}{}

\newcommand{\WSpartitionNarrowL}{
\begin{minipage}[t]{2.0in}
\begin{tabbing}
id \= id \= \kill
{\bf \color{blue} Partition} 
\partitioningsL \+ \\
{\bf \color{blue} where } 
\begin{minipage}[t]{2in}
\partitionsizesL 
\end{minipage}
\end{tabbing}
\end{minipage}
}

\newcommand{\WSpartitionNarrowR}{
\begin{minipage}[t]{2.0in}
\begin{tabbing}
id \= id \= \kill
{\bf Partition} 
\partitioningsR \+ \\
{\bf where} 
\begin{minipage}[t]{2in}
\partitionsizesR 
\end{minipage}
\end{tabbing}
\end{minipage}
}


\newcommand{\WSrepartitionNarrowL}{
\begin{minipage}[t]{2.05in}
{\bf \color{blue} Repartition}
\begin{tabbing}
i \= i \= \+ \kill
\repartitioningsL \+ \\
{\bf \color{blue} where}
\begin{minipage}[t]{2in}
\repartitionsizesL
\end{minipage}
\end{tabbing}
\end{minipage}
}


\newcommand{\WSrepartitionNarrowR}{
\begin{minipage}[t]{2.05in}
{\bf \color{blue} Repartition}
\begin{tabbing}
i \= i \= \+ \kill
\repartitioningsR \+ \\
{\bf \color{blue} where}
\begin{minipage}[t]{2in}
\repartitionsizesR
\end{minipage}
\end{tabbing}
\end{minipage}
}


\newcommand{\WSblocksizeL}{
\ifthenelse{ \equal{\blocksizeL}{1}}{}
{%
\ifthenelse{ \equal{\blocksizeL}{blank} }{}
}
{{\bf \color{blue} Determine block size $ \blocksizeL $}} 
}

\newcommand{\WSblocksizeR}{
\ifthenelse{ \equal{\blocksizeR}{1} }{}
{%
\ifthenelse{ \equal{\blocksizeR}{blank} }{}
}
{{\bf \color{blue} Determine block size $ \blocksizeR $}} 
}


\newcommand{\WSmoveboundaryNarrowL}{
\begin{minipage}[t]{2.05in}
{\bf \color{blue} Continue with}
\begin{tabbing}
i \= \+ \kill
\moveboundariesL 
\end{tabbing}
\end{minipage}
}



\newcommand{\WSmoveboundaryNarrowR}{
\begin{minipage}[t]{2.05in}
{\bf Continue with}
\begin{tabbing}
i \= \+ \kill
\moveboundariesR 
\end{tabbing}
\end{minipage}
}


\newcommand{\WSupdateL}{
\updateL
}

\newcommand{\WSupdateR}{
\updateR
}


\newcommand{\FlaAlgorithmTwo}{
\begin{center}
\begin{tabular}{| p{3.0in} | @{}c@{} | p{3.0in} |} 
\cline{1-1} \cline{3-3}
% {\bf \color{blue} Algorithm:} 
$\routinenameL$
&
~
&
% {\bf \color{blue} Algorithm:} 
$\routinenameR$
\\ \cline{1-1} \cline{3-3}
\begin{tabular}{@{}l}
\WSpartitionNarrowL
\end{tabular}
&
&
\begin{tabular}{@{}l}
\WSpartitionNarrowR
\end{tabular}
\\
{\bf \color{blue} while} \WSguard { \bf \color{blue} do} 
&
&
{\bf \color{blue} while} \WSguard { \bf \color{blue} do} \\
\ifthenelse{ \equal{\blocksizeL}{blank} }{
\ifthenelse{ \equal{\blocksizeR}{blank} }{}
{
\ \hspace{0.0in} \WSblocksizeL
&
&
\ \hspace{0.0in} \WSblocksizeR
\\}
}
\ \hspace{0.0in} \WSrepartitionNarrowL 
&
&
\ \hspace{0.0in} \WSrepartitionNarrowR 
\\
{\hspace{0.0in} \FlaComputeSection{2.75in} }
&
&
{\hspace{0.0in} \FlaComputeSection{2.75in} }
\\
{\hspace{0.0in} \WSupdateL} 
&
&
{\hspace{0.0in} \WSupdateR} 
\\
{\hspace{0.0in} \FlaComputeSection{2.75in} }
&
&
{\hspace{0.0in} \FlaComputeSection{2.75in} }
\\
{\ \hspace{0.0in} \WSmoveboundaryNarrowL} 
&
&
{\ \hspace{0.0in} \WSmoveboundaryNarrowR} 
\\
{{\bf \color{blue} endwhile}} 
&
&
{{\bf \color{blue} endwhile}} 
\\ \cline{1-1} \cline{3-3}
\end{tabular}
\end{center}
}


==> macros.tex <==
% THEOREMS -------------------------------------------------------

\setlength{\topsep}{0pt}
% \newtheorem{algorithm}{Algorithm}[chapter] % already in SIAM macros
% \newtheorem{lemma}{Lemma}[section] % already in SIAM macros
% \newtheorem{corollary}{Corollary}[chapter] % already in SIAM macros
% \newtheorem{example}{Example} % already in SIAM macros
% \newtheorem{theorem}{Theorem}[chapter] % already in SIAM macros
% \newtheorem{definition}{Definition}[chapter] % already in SIAM macros
% \newtheorem{definition}{Definition} % already in SIAM macros
\newtheorem{remark}{Remark}[section]
\newtheorem{exercise}{Exercise}[section]
\renewenvironment{proof}{\noindent
{\bf Proof:}}
{\hfill {\bf endofproof}}

\newenvironment{boxedexample}{
\noindent
\newline
\begin{boxedminipage}[t]{\textwidth}
\addtocounter{ourexample}{1}%
{\bf Example \thechapter.\theourexample.}
\em
}
{
\end{boxedminipage}
}

\newenvironment{boxedexercise}{
\noindent
\newline
\begin{boxedminipage}[t]{\textwidth}
\begin{exercise}
}
{
\end{exercise}
\end{boxedminipage}
}

\newenvironment{boxit}{
\noindent
\newline
\begin{boxedminipage}[t]{\textwidth}
}
{
\end{boxedminipage}
}

\newenvironment{boxedremark}{%
\noindent
\begin{boxedminipage}[t]{\textwidth}
\begin{remark}
}
{
\end{remark}
\end{boxedminipage}
}

% \newcounter{remark}
\newcounter{mydefinition}

%%\newenvironment{boxedremark}{%
%%%
%%\noindent
%%\begin{boxedminipage}[t]{\textwidth}
%%\addtocounter{remark}{1}%
%%{\bf Remark \thechapter.\theremark.}
%%\em
%%}
%%{
%%\end{boxedminipage}
%%}


\newenvironment{notetoexpert}{%
\noindent
\newline
\begin{boxedminipage}[t]{\textwidth}
\addtocounter{remark}{1}%
{\bf Note to the skeptical expert.}
\em
}
{
\end{boxedminipage}
}


\newenvironment{boxeddefinition}{%
\noindent
\newline
\begin{boxedminipage}[t]{\textwidth}
\addtocounter{mydefinition}{1}%
{\bf Definition \chapter.\themydefinition.}
\em
}
{
\end{boxedminipage}
}

\newcommand{\eop}{
{\bf endofproof}
}

\newcommand{\I}{\mathbb{I}}
\renewcommand{\R}{\mathbb{R}}
\renewcommand{\C}{\mathbb{C}}
\renewcommand{\S}{\mathbb{S}}

\newcommand{\Rm}{\R^{m}}
\newcommand{\Rn}{\R^{n}}
\newcommand{\Rk}{\R^{k}}


\newcommand{\Cm}{\C^{m}}
\newcommand{\Cn}{\C^{n}}
\newcommand{\Ck}{\C^{k}}

\newcommand{\Rmxm}{\R^{m \times m}}
\newcommand{\Rnxn}{\R^{n \times n}}
\newcommand{\Rmxn}{\R^{m \times n}}
\newcommand{\Rnxm}{\R^{n \times m}}

\newcommand{\Rmxk}{\R^{m \times k}}
\newcommand{\Rkxn}{\R^{k \times n}}
\newcommand{\Rnxk}{\R^{n \times k}}
\newcommand{\Rkxk}{\R^{k \times k}}

\newcommand{\Cmxm}{\C^{m \times m}}
\newcommand{\Cnxn}{\C^{n \times n}}
\newcommand{\Cmxn}{\C^{m \times n}}
\newcommand{\Cnxm}{\C^{n \times m}}

\newcommand{\Cmxk}{\C^{m \times k}}
\newcommand{\Ckxn}{\C^{k \times n}}
\newcommand{\Cnxk}{\C^{n \times k}}
\newcommand{\Ckxk}{\C^{k \times k}}

\newcommand{\Sm}{\S^{m}}
\newcommand{\Sn}{\S^{n}}
\newcommand{\Sk}{\S^{k}}
\newcommand{\Sonexm}{\S^{1 \times m}}

\newcommand{\Smxm}{\S^{m \times m}}
\newcommand{\Snxn}{\S^{n \times n}}
\newcommand{\Smxn}{\S^{m \times n}}
\newcommand{\Snxm}{\S^{n \times m}}

\newcommand{\Smxk}{\S^{m \times k}}
\newcommand{\Skxn}{\S^{k \times n}}
\newcommand{\Snxk}{\S^{n \times k}}

\newcommand{\alert}{!!!}
\newcommand{\row}[1]{\check{#1}}
\newcommand{\tr}[1]{{#1}^{\mathrm{T}}}
\newcommand{\tri}[1]{{#1}^{\mathrm{-T}}}
\newcommand{\tc}[1]{{#1}^{\mathrm{H}}}
\newcommand{\op}[1]{{\mathrm{op}(#1)}}

\newcommand{\TrLw}[1]{\mathrm{TrLw}(#1)}
\newcommand{\TrUp}[1]{\mathrm{TrUp}(#1)}
\newcommand{\SyLw}[1]{\mathrm{SyLw}(#1)}
\newcommand{\SyUp}[1]{\mathrm{SyUp}(#1)}
\newcommand{\HeLw}[1]{\mathrm{HeLw}(#1)}
\newcommand{\HeUp}[1]{\mathrm{HeUp}(#1)}

\newcommand{\cF}{{\cal{F}}}
\newcommand{\cG}{{\cal{G}}}
\newcommand{\cH}{{\cal{H}}}

\newcommand{\defcolvector}[2]{
\left( 
\begin{array}{c}
#1_0 \\  \hline
\vdots \\ \hline
#1_{#2-1}
\end{array} 
\right)
}

\newcommand{\defcolvectoratones}[2]{
\left( 
\begin{array}{c}
#1_1 \\ 
#1_2 \\ 
\vdots \\ 
#1_{#2}
\end{array} 
\right)
}

\newcommand{\defrowvector}[2]{
\left(
\begin{array}{c | c | c }
#1_0 & \ldots & #1_{#2-1}
\end{array}
\right)
}

\newcommand{\defmatrix}[3]{
\left( 
\begin{array}{c | c | c }
#1_{00}     & \cdots & #1_{0,#3-1} \\ 
\vdots      & \ddots       &\vdots    \\ 
#1_{#2-1,0} & \cdots & #1_{#2-1,#3-1} \\ 
\end{array} 
\right)
}

\newcommand{\unit}{\mbox{\bf u}}

% \newcommand{\sign}{\mbox{\rm sign}}

% \newcommand{\Chol}[1]{\mbox{\sc Chol}( #1 )}
\newcommand{\Chol}[1]{\Gamma( #1 )}
\newcommand{\QR}[1]{\mbox{\sc QR}( #1 )}
\newcommand{\LU}[1]{\mbox{\sc LU}( #1 )}
\newcommand{\LUpiv}[1]{\mbox{\sc LUpiv}( #1 )}
\newcommand{\tril}[1]{\mbox{\sc tril}\left( #1 \right)}
\newcommand{\triu}[1]{\mbox{\sc triu}( #1 )}
\newcommand{\trilu}[1]{\mbox{\sc trilu}( #1 )}
\newcommand{\triuu}[1]{\mbox{\sc triuu}( #1 )}
\newcommand{\housev}[1]{\mbox{\sc Housev}( #1 )}

% Operation names
\newcommand{\scal}{\mbox{\sc scal}}
\newcommand{\add}{\mbox{\sc add}}
\newcommand{\sdot}{\mbox{\sc dot}}
\newcommand{\sapdot}{\mbox{\sc apdot}}
\newcommand{\saxpy}{\mbox{\sc axpy}}
\newcommand{\matvec}{\mbox{\sc gemv}}
\newcommand{\vecmat}{\mbox{\sc gevm}}
\newcommand{\rankone}{\mbox{\sc ger}}
\newcommand{\trsv}{\mbox{\sc trsv}}
\newcommand{\matmat}{\mbox{\sc gemm}}
\newcommand{\symm}{\mbox{\sc symm}}
\newcommand{\trmm}{\mbox{\sc trmm}}
\newcommand{\trsm}{\mbox{\sc trsm}}
\newcommand{\syrk}{\mbox{\sc syrk}}
\newcommand{\ger}{\mbox{\sc ger}}

\newcommand{\gemm}{\mbox{\sc gemm}}

% Products
\newcommand{\matlab}{\mbox{\sc Matlab}}
\newcommand{\octave}{\mbox{\sc Octave}}
\newcommand{\labview}{\mbox{\sc LabView}}
\newcommand{\haskell}{\mbox{\sc Haskell}}
\newcommand{\mathematica}{\mbox{\sc Mathematica}}
\newcommand{\ieee}{\mbox{\sc ieee}}

\newcommand{\GFLOPS}{\mbox{GFLOPS}}

%% \newcommand{\blkblk}{\mbox{\sc gebb}}
%% \newcommand{\blkpan}{\mbox{\sc gebp}}
%% \newcommand{\panblk}{\mbox{\sc gepb}}
%% \newcommand{\pandot}{\mbox{\sc gepdot}}
%% \newcommand{\panpan}{\mbox{\sc gepp}}
%% \newcommand{\matpan}{\mbox{\sc gemp}}
%% \newcommand{\panmat}{\mbox{\sc gepm}}
%% \newcommand{\panvec}{\mbox{\sc gepv}}

\newcommand{\blkblk}{\mbox{\sc gemm\_bb}}
\newcommand{\blkpan}{\mbox{\sc gemm\_bp}}
\newcommand{\panblk}{\mbox{\sc gemm\_pb}}
\newcommand{\pandot}{\mbox{\sc gemm\_pd}}
\newcommand{\panpan}{\mbox{\sc gemm\_pp}}
\newcommand{\matpan}{\mbox{\sc gemm\_mp}}
\newcommand{\panmat}{\mbox{\sc gemm\_pm}}
\newcommand{\panvec}{\mbox{\sc gemm\_pv}}


\newcommand{\chol}{\mbox{\sc chol}}
\newcommand{\lu}{\mbox{\sc lu}}

\newcommand{\Aaux}{ A_{\rm aux}}
\newcommand{\Baux}{ B_{\rm aux}}
\newcommand{\Caux}{ C_{\rm aux}}

\newcommand{\resetcounters}{
\setcounter{remark}{0}
\setcounter{mydefinition}{0}
}


